Unsupervised Object Discovery: A Comprehensive Survey and Unified Taxonomy

Unsupervised object discovery is commonly interpreted as the task of localizing and/or categorizing objects in visual data without the need for labeled examples. While current object recognition methods have proven highly effective for practical applications, the ongoing demand for annotated data in real-world scenarios drives research into unsupervised approaches. Furthermore, existing literature in object discovery is both extensive and diverse, posing a significant challenge for researchers that aim to navigate and synthesize this knowledge. Motivated by the evidenced interest in this avenue of research, and the lack of comprehensive studies that could facilitate a holistic understanding of unsupervised object discovery, this survey conducts an in-depth exploration of the existing approaches and systematically categorizes this compendium based on the tasks addressed and the families of techniques employed. Additionally, we present an overview of common datasets and metrics, highlighting the challenges of comparing methods due to varying evaluation protocols. This work intends to provide practitioners with an insightful perspective on the domain, with the hope of inspiring new ideas and fostering a deeper understanding of object discovery approaches.

==> dataset_hist.tex <==
\pgfplotsset{width=12cm}

\begin{figure}
\begin{center}
\begin{tikzpicture}
\tikzstyle{every node}=[font=\tiny]
\begin{axis}[
ybar stacked,
bar width=8pt,
nodes near coords,
enlargelimits=0.05,
legend style={at={(0.7,0.95)},
anchor=north,legend columns=1},
ylabel={\# of Methods},
symbolic x coords={{MNIST | MNIST variants},{Fashion-MNIST},SIVAL,SVHN,
{PASCAL VOC 2007}, {PASCAL VOC 2012}, {MS COCO 2014}, {MS COCO 2017}, {CIFAR-10}, {CIFAR-100}, {STL-10}, OpenImages, iCoseg, {CUB-200-2011}, 
{Object Discovery}, {ImageNet Subsets}, {Stanford Dogs}, {Stanford Cars}, Omniglot, {Simple Shapes}, {CLEVR | CLEVR variants}, {Multi-dSprites}, Tetrominoes, {Objects Room}, {Atari Games}, {Custom Datasets},
{Other Datasets}
},
xtick=data,
x tick label style={rotate=45,anchor=east},
]
\addplot+ [ybar, fill=softyellow, draw=gray, text=black] coordinates {
({MNIST | MNIST variants},7) 
({Fashion-MNIST},1)
(SIVAL,0) 
(SVHN,3) 
({PASCAL VOC 2007},0) 
({PASCAL VOC 2012},0) 
({MS COCO 2014},0) 
({MS COCO 2017},1) 
({CIFAR-10},6) 
({CIFAR-100},5) 
({STL-10},6) 
(OpenImages,0) 
(iCoseg,1) 
({CUB-200-2011},1) 
({Object Discovery},0) 
({ImageNet Subsets},1) 
({Stanford Dogs},1) 
({Stanford Cars},1) 
(Omniglot,1) 
({Simple Shapes},0) 
({CLEVR | CLEVR variants},0) 
({Multi-dSprites},0) 
(Tetrominoes,0) 
({Objects Room},0) 
({Atari Games},0) 
({Custom Datasets},0) 
({Other Datasets},3)};

\addplot+ [ybar, fill=softorange, draw=gray, text=black] coordinates {
({MNIST | MNIST variants},11) 
({Fashion-MNIST},0)
(SIVAL,0) 
(SVHN,0) 
({PASCAL VOC 2007},8) 
({PASCAL VOC 2012},3) 
({MS COCO 2014},1) 
({MS COCO 2017},1)
({CIFAR-10},0) 
({CIFAR-100},0) 
({STL-10},0) 
(OpenImages,1) 
(iCoseg,0) 
({CUB-200-2011},2) 
({Object Discovery},5) 
({ImageNet Subsets},3) 
({Stanford Dogs},1) 
({Stanford Cars},1) 
(Omniglot,1) 
({Simple Shapes},2) 
({CLEVR | CLEVR variants},8) 
({Multi-dSprites},7) 
(Tetrominoes,2) 
({Objects Room},4) 
({Atari Games},3) 
({Custom Datasets},12) 
({Other Datasets},15)};

\addplot+ [ybar, fill=softred, draw=gray, text=black] coordinates {
({MNIST | MNIST variants},4) 
({Fashion-MNIST},1)
(SIVAL,2) 
(SVHN,3) 
({PASCAL VOC 2007},4) 
({PASCAL VOC 2012},2) 
({MS COCO 2014},2) 
({MS COCO 2017},0)
({CIFAR-10},2) 
({CIFAR-100},0) 
({STL-10},0) 
(OpenImages,0) 
(iCoseg,1) 
({CUB-200-2011},0) 
({Object Discovery},2) 
({ImageNet Subsets},2) 
({Stanford Dogs},0) 
({Stanford Cars},0) 
(Omniglot,0) 
({Simple Shapes},0) 
({CLEVR | CLEVR variants},1) 
({Multi-dSprites},1) 
(Tetrominoes,1) 
({Objects Room},0) 
({Atari Games},0) 
({Custom Datasets},3) 
({Other Datasets},2)};


\legend{Categorization, Localization, Categorization+Localization}
\end{axis}
\end{tikzpicture}
\end{center}
\end{figure}


==> fig_levels.tex <==
% Simulation approaches versus abstraction levels
% Author: Valeria Borodin

\usetikzlibrary{positioning,shadows.blur}
%\renewcommand{\labelitemi}{\ding{112}}
%font       = \sffamily\bfseries, 
% blur shadow = {shadow blur steps = 5}

\begin{center}
\begin{tikzpicture}
  \tikzset{
    box/.style = { 
        rounded corners = 2pt, align = left, font = \tiny, text width = 2cm, blur shadow = {shadow blur steps = 15} },
    box_single_image_aware/.style = { draw = gray!80, dashed,
        rounded corners = 2pt, align = center, font = \tiny, fill = softyellow },
    box_mult_patch_agnostic/.style = { draw = black!80,
        rounded corners = 2pt, align = center, font = \tiny, fill = softblue },
    box_mult_patch_aware/.style = { draw = black!80, dashed,
        rounded corners = 2pt, align = center, font = \tiny, fill = softblue },
    box_single_patch_agnostic/.style = { draw = black!80,
        rounded corners = 2pt, align = right, font = \tiny, fill = softorange},
    box_single_patch_aware/.style = { draw = black!80, dashed,
        rounded corners = 2pt, align = center, font = \tiny, fill = softorange },
    box_mult_pixel_agnostic/.style = { draw = black!80, 
        rounded corners = 2pt, align = center, font = \tiny, fill = softpurple },
    box_mult_pixel_aware/.style = { draw = black!80, dashed,
        rounded corners = 2pt, align = center, font = \tiny, fill = softpurple },
    box_single_pixel_agnostic/.style = { draw = black!80,
        rounded corners = 2pt, align = right, font = \tiny, fill = softred},
    box_legend_b/.style = { draw = black!80, text width = 2cm, 
        line width = 0.5pt, rounded corners = 2pt, align = center, font = \tiny},
    box_legend_m/.style = { draw = black!80, dashed, text width = 2cm, 
        line width = 0.5pt, rounded corners = 2pt, align = center, font = \tiny},
    legend_h/.style = { font = \small, align = center},
    legend_v/.style = { font = \small, align = center, rotate = 90},
  }
  
  \node [shade,
    text width = 0.91\textwidth, top color = white, bottom color = white,
    text = black, font         = \small] (A)
    {\\ \vspace{.55\textwidth}};
  
  % A11 - Multiple Objects - Image Level
  %% EMPTY CELL
  
  % A21 - Single Object - Image Level
  \node [box_single_image_aware, below left = 5.5cm and -0.75cm of A.north west, anchor = north west] (A21_aw_1){AAE};
  \node [box_single_image_aware, right = 0 of A21_aw_1] (A21_aw_2){ADC};
  \node [box_single_image_aware, right = 0 of A21_aw_2] (A21_aw_3){DAC};
  \node [box_single_image_aware, below = 0 of A21_aw_1.south west, anchor=north west] (A21_aw_4){DTI};
  \node [box_single_image_aware, right = 0 of A21_aw_4] (A21_aw_5){FineGAN};
  \node [box_single_image_aware, below = 0 of A21_aw_4.south west, anchor=north west] (A21_aw_6){GMVAE};
  \node [box_single_image_aware, right = 0 of A21_aw_6] (A21_aw_7){IIC};
  \node [box_single_image_aware, right = 0 of A21_aw_7] (A21_aw_8){IMSAT};
  \node [box_single_image_aware, below = 0 of A21_aw_6.south west, anchor=north west] (A21_aw_9){SCAN};
  \node [box_single_image_aware, right = 0 of A21_aw_9] (A21_aw_10){TwoFoldOp};
  
  % A12 - Multiple Objects - Patch Level
  \node [box_mult_patch_agnostic, below left = 0cm and -5cm of A.north west, anchor = north west] (A12_ag_1){AIR};
  \node [box_mult_patch_agnostic, right = 0cm of A12_ag_1] (A12_ag_2){GNM};
  \node [box_mult_patch_agnostic, right = 0cm of A12_ag_2] (A12_ag_3){GSGNs};
  \node [box_mult_patch_agnostic, right = 0cm of A12_ag_3] (A12_ag_4){OLM};
  \node [box_mult_patch_agnostic, below = 0 of A12_ag_1.south west, anchor = north west] (A12_ag_5){PatchNet};
  \node [box_mult_patch_agnostic, right = 0cm of A12_ag_5] (A12_ag_6){rOSD};
  \node [box_mult_patch_agnostic, right = 0cm of A12_ag_6] (A12_ag_7){SCALOR};
  \node [box_mult_patch_agnostic, below = 0 of A12_ag_5.south west, anchor = north west] (A12_ag_8){SPACE};
  \node [box_mult_patch_agnostic, right = 0cm of A12_ag_8] (A12_ag_9){SPAIR};
  \node [box_mult_patch_agnostic, right = 0cm of A12_ag_9] (A12_ag_10){SQAIR};
  \node [box_mult_patch_agnostic, below = 0 of A12_ag_8.south west, anchor = north west] (A12_ag_11){SuPAIR};
  
  \node [box_mult_patch_aware, below = 0.25cm of A12_ag_11.south west, anchor = north west] (A12_aw_1){bMCL};
  \node [box_mult_patch_aware, right = 0 of A12_aw_1] (A12_aw_2){GMAIR};
  \node [box_mult_patch_aware, right = 0 of A12_aw_2] (A12_aw_3){LOD};
  \node [box_mult_patch_aware, below = 0 of A12_aw_1.south west, anchor = north west] (A12_aw_4){LOST};
  \node [box_mult_patch_aware, right = 0 of A12_aw_4] (A12_aw_5){StampNet};
  
  % A22 - Single Object - Patch Level
  \node [box_single_patch_agnostic, below left = 5.5cm and -5cm of A.north west, anchor = north west] (A22_ag_1){UODLWild};
  \node [box_single_patch_agnostic, right = 0 of A22_ag_1] (A22_ag_2){DDT};
  \node [box_single_patch_agnostic, right = 0 of A22_ag_2] (A22_ag_3){CoLocFW};
  \node [box_single_patch_agnostic, below = 0 of A22_ag_1.south west, anchor = north west] (A22_ag_4){CoLocGDP};
  \node [box_single_patch_agnostic, right = 0 of A22_ag_4] (A22_ag_5){CoLocCSD};
  \node [box_single_patch_agnostic, right = 0 of A22_ag_5] (A22_ag_6){OSD};
  \node [box_single_patch_agnostic, below = 0 of A22_ag_4.south west, anchor = north west] (A22_ag_7){CoLocRWI};
  
  \node [box_single_patch_aware, below = 0.25cm of A22_ag_7.south west, anchor = north west](A22_aw_1){UODSphClust};
   
  % A13 - Multiple Objects - Pixel Level 
  \node [box_mult_pixel_agnostic, below left = 0cm and -10cm of A.north west, anchor = north west] (A13_ag_1){CST-VAE};
  \node [box_mult_pixel_agnostic, right = 0cm of A13_ag_1] (A13_ag_2){DeepCO3};
  \node [box_mult_pixel_agnostic, right = 0cm of A13_ag_2] (A13_ag_3){DMFC};
  \node [box_mult_pixel_agnostic, below = 0 of A13_ag_1.south west, anchor = north west] (A13_ag_4){DSM};
  \node [box_mult_pixel_agnostic, right = 0cm of A13_ag_4] (A13_ag_5){EfficientMORL};
  \node [box_mult_pixel_agnostic, right = 0cm of A13_ag_5] (A13_ag_6){GENESIS};
  \node [box_mult_pixel_agnostic, below = 0 of A13_ag_4.south west, anchor = north west] (A13_ag_7){GenesisV2};
  \node [box_mult_pixel_agnostic, right = 0cm of A13_ag_7] (A13_ag_8){CoAttnCNN};
  \node [box_mult_pixel_agnostic, right = 0cm of A13_ag_8] (A13_ag_10){IODINE};
  \node [box_mult_pixel_agnostic, below = 0 of A13_ag_7.south west, anchor = north west] (A13_ag_11){CoSegECEM};
  \node [box_mult_pixel_agnostic, right = 0cm of A13_ag_11] (A13_ag_12){MONet};
  \node [box_mult_pixel_agnostic, right = 0cm of A13_ag_12] (A13_ag_13){MulMON};
  \node [box_mult_pixel_agnostic, below = 0 of A13_ag_11.south west, anchor = north west] (A13_ag_14){N-EM};
  \node [box_mult_pixel_agnostic, right = 0cm of A13_ag_14] (A13_ag_15){PSGNet};
  \node [box_mult_pixel_agnostic, right = 0cm of A13_ag_15] (A13_ag_16){R-NEM};
  \node [box_mult_pixel_agnostic, below = 0 of A13_ag_14.south west, anchor = north west] (A13_ag_17){SelfMask};
  \node [box_mult_pixel_agnostic, right = 0cm of A13_ag_17] (A13_ag_18){Slot Attention};
  \node [box_mult_pixel_agnostic, right = 0cm of A13_ag_18] (A13_ag_19){SRN};
  \node [box_mult_pixel_agnostic, below = 0 of A13_ag_17.south west, anchor = north west] (A13_ag_20){TAGGER};
  \node [box_mult_pixel_agnostic, right = 0cm of A13_ag_20] (A13_ag_21){uORF};
  \node [box_mult_pixel_agnostic, right = 0cm of A13_ag_21] (A13_ag_22){LMIO};
  \node [box_mult_pixel_agnostic, right = 0cm of A13_ag_22] (A13_ag_23){GMIOO};
  \node [box_mult_pixel_agnostic, right = 0cm of A13_ag_23] (A13_ag_24){CoSand};
  \node [box_mult_pixel_agnostic, right = 0cm of A13_ag_24] (A13_ag_25){COMP};

  \node [box_mult_pixel_aware, below = 0.25cm of A13_ag_20.south west, anchor = north west] (A13_aw_1){DPR-CAE};
  \node [box_mult_pixel_aware, right = 0 of A13_aw_1] (A13_aw_2){DTI-Sprites};
  \node [box_mult_pixel_aware, right = 0 of A13_aw_2] (A13_aw_3){ECON};
  \node [box_mult_pixel_aware, right = 0cm of A13_aw_3] (A13_aw_4){IIC-sec};
  \node [box_mult_pixel_aware, below = 0 of A13_aw_1.south west, anchor = north west] (A13_aw_5){MarioNette};
  \node [box_mult_pixel_aware, right = 0cm of A13_aw_5] (A13_aw_6){MaskContrast};
  \node [box_mult_pixel_aware, right = 0cm of A13_aw_6] (A13_aw_7){PiCIE};
  \node [box_mult_pixel_aware, below = 0 of A13_aw_5.south west, anchor = north west] (A13_aw_8){SCAE};
  \node [box_mult_pixel_aware, right = 0cm of A13_aw_8] (A13_aw_9){SegDiscover};
  
  % A23 - Single Object - Pixel Level 
  \node [box_single_pixel_agnostic, below left = 5.5cm and -10cm of A.north west, anchor = north west] (A23_ag_1){UVISAM};
  \node [box_single_pixel_agnostic, right = 0 of A23_ag_1] (A23_ag_2){CP-GAN};
  \node [box_single_pixel_agnostic, right = 0 of A23_ag_2] (A23_ag_3){DeepUSPS};
  \node [box_single_pixel_agnostic, below = 0 of A23_ag_1.south west, anchor=north west] (A23_ag_4){DFF};
  \node [box_single_pixel_agnostic, right = 0 of A23_ag_4] (A23_ag_5){DRC};
  \node [box_single_pixel_agnostic, right = 0 of A23_ag_5] (A23_ag_6){CoSegGuid};
  \node [box_single_pixel_agnostic, right = 0 of A23_ag_6] (A23_ag_7){ReDo};
  \node [box_single_pixel_agnostic, right = 0 of A23_ag_7] (A23_ag_8){SGC3};
  \node [box_single_pixel_agnostic, below = 0 of A23_ag_4.south west, anchor=north west] (A23_ag_9){CoSegHueSat};
  \node [box_single_pixel_agnostic, right = 0 of A23_ag_9] (A23_ag_10){TokenCut};
  \node [box_single_pixel_agnostic, right = 0 of A23_ag_10] (A23_ag_11){UnsupOD};
  \node [box_single_pixel_agnostic, below = 0 of A23_ag_9.south west, anchor=north west] (A23_ag_12){SegLSGM};
  \node [box_single_pixel_agnostic, right = 0 of A23_ag_12] (A23_ag_13){SSW};
  \node [box_single_pixel_agnostic, right = 0 of A23_ag_13] (A23_ag_14){USDNoisyLbl};
  \node [box_single_pixel_agnostic, right = 0 of A23_ag_14] (A23_ag_15){SegSwap};
  \node [box_single_pixel_agnostic, right = 0 of A23_ag_15] (A23_ag_16){OD};
  
  
  % axis legends
  \node [legend_v, above left = -1.0cm and 0.1cm of A](L3)
    {Multiple\\Objects};
  \node [legend_v, below left = 3.0cm and 0.9cm of L3] (L2)
    {Single\\Object};

  \node [legend_h, below left = 0.1cm and -3cm of A] (C1) 
    {Image-Level\\(Entire Image)};
  \node [legend_h, right = 2.75cm of C1] (C2) 
    {Patch-Level\\(Bounding-Box)};
  \node [legend_h, right = 3cm of C2] (C3) 
    {Pixel-Level\\(Mask)};
 
  \path [draw, <->, >=latex, line width = 2pt, gray ]
     (A.south west)  + (0cm,0) coordinate(y) -- (y|-A.north);
  \path [draw, <->, >=latex, line width = 2pt, gray ]
     (A.south west)  + (0cm,0cm) coordinate(x) -- (x-|A.east);
     
  \matrix [draw, gray, rounded corners = 2pt, line width = 1.5pt, row sep=1mm, below right = 0cm and 0.25cm of A.north west]{
    \node [box_legend_b] {Class-Agnostic};\\
    \node [box_legend_m] {Class-Aware};\\
  };
\end{tikzpicture}
\end{center}

==> tables/table_overview_all_onepage.tex <==
\let\conftitle\footnotesize

\begin{longtable}[]
\small
\resizebox{\columnwidth}{!}{%
%\setlength{\aboverulesep}{0pt} % Reduce space above rules
%\setlength{\belowrulesep}{0pt} % Reduce space below rules
\begin{tabular}{clcccccc}
%>{\kern-\tabcolsep}
%\begin{tabular}{@{}clcccccc@{}}
%\toprule
\toprule
%\specialrule{*}{0pt}{0pt}
\multicolumn{8}{c}{\cellcolor[HTML]{DDDDDD} {\textbf{Methods}}}                                 \\ \midrule
   &
  Method &
  \begin{tabular}[c]{@{}c@{}}Pub.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Year\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Model\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Optimization\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Representation\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Learning\end{tabular} \\ \midrule

%% ----------------------------------------------------------------------------------------%%
%% --                                  CLUSTERING                                        --%%
%% ----------------------------------------------------------------------------------------%%

\cellcolor{colorclust}& DEC & \conftitle{ICML} & 2015 & Repr. Learning/Probab. Clust. & Backprop/Refinement (k-means) & Learned & Target distrib.  \\ [-\arrayrulewidth]

\rowcolor{rowbackground}
 \cellcolor{colorclust}& AAE	& \conftitle{ARXIV} & 2016 & Autoencoder/Adversarial Net & Backprop/Adversarial training & Learned & Img. reconstruction  \\ [-\arrayrulewidth]
\cellcolor{colorclust}& JULE & \conftitle{CVPR} & 2016 & Rec. CNN/Agglom. Clust. & Backprop/Greedy Search & Learned & Weighted triplet loss  \\ [-\arrayrulewidth]

\rowcolor{rowbackground}
\cellcolor{colorclust} & DAC & \conftitle{ICCV} & 2017 & Binary Pairwise-Classifier & Backprop/Adaptive training & Pretrained & Pairwise similarities  \\ [-\arrayrulewidth]
\cellcolor{colorclust} & GMVAE & \conftitle{ICLR} & 2017 & Variational autoencoder & Backprop/Variational inference & Learned & ELBO  \\ [-\arrayrulewidth]

\rowcolor{rowbackground}
\cellcolor{colorclust} & IMSAT & \conftitle{ICML} & 2017 & discrete repr. learning & Backprop/Information Theory & Pretrained & Transformations/MI  \\ [-\arrayrulewidth]
\cellcolor{colorclust} & ADC	& \conftitle{GCPR} & 2018 & Classification network & Backprop/Associative clustering & Learned & Transform. invariant loss  \\ [-\arrayrulewidth]

\rowcolor{rowbackground}
\cellcolor{colorclust} & FineGAN & \conftitle{CVPR} & 2019 & Hierarchical GAN & Backprop/Adversarial training & Learned & Adversarial + MI  \\ [-\arrayrulewidth]
\cellcolor{colorclust} & IIC & \conftitle{ICCV} & 2019 & Classification network & Backprop/Information Theory & Learned & Transformations/MI  \\ [-\arrayrulewidth]

\rowcolor{rowbackground}
\cellcolor{colorclust} & DTI-GMM	& \conftitle{NIPS} & 2020 & Transformation Prediction & Backprop/EM & - & Transform. invariant loss  \\ [-\arrayrulewidth]
\cellcolor{colorclust} & SCAN & \conftitle{ECCV} & 2020 & Repr. learning+Classif. net. & Backprop/Nearest neighbors & Learned & Semantic clustering loss \\ [-\arrayrulewidth]

\rowcolor{rowbackground}
\multirow[c]{-12}{0.7em}{\cellcolor{colorclust}
\begin{sideways}\textcolor{white}{\textbf{CLUSTERING}}\end{sideways}} & TwoFoldOp & \conftitle{NEUROC} & 2022 & Repr. learning+Classif. net. & Backprop/Alternating loss (EM-like) & Learned & Clust. loss/ KL aug.  \\ [-\arrayrulewidth]

%% ----------------------------------------------------------------------------------------%%
%% --                                  LOCALIZATION                                      --%%
%% ----------------------------------------------------------------------------------------%%
\midrule

\cellcolor{colorloc} & CL-FWA &  \conftitle{ECCV} & 2014 & Combinatorial/Quad. progr. &  Frank-Wolfe algorithm & hand-crafted & x \\ [-\arrayrulewidth]

\rowcolor{rowbackground}
\cellcolor{colorloc} & CL-CSD &  \conftitle{ECCV} & 2016 & Prop. Scoring/Graph-based & SGD/Graph cuts & pretrained & x  \\ [-\arrayrulewidth]
\cellcolor{colorloc} & OLM &  \conftitle{TIP} & 2020 & Pattern Mining/Transact. & Data mining/CNN layers & pretrained & x  \\ [-\arrayrulewidth]

\rowcolor{rowbackground}
\cellcolor{colorloc} & LOD &  \conftitle{NIPS} & 2021 & Ranking/Graph-based & Quadratic op./PageRank & pretrained & x \\ [-\arrayrulewidth]
\cellcolor{colorloc} & LOST &  \conftitle{BMVC} & 2021 &  &  & pretrained & x \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorloc} & PatchNet &  \conftitle{ARXIV} & 2021 & VAE/Pattern Space & Backprop/Clustering & learned & contrastive   \\ [-\arrayrulewidth]
\cellcolor{colorloc} & TokenCut &  \conftitle{CVPR} & 2022 & Graph-based Spectral & Normalized cut & pretrained & x  \\ [-\arrayrulewidth]


\rowcolor{rowbackground}
\cellcolor{colorloc} & CL-CSD &  \conftitle{ECCV} & 2016 & Prop. Scoring/Graph-based & SGD/Graph cuts & pretrained & x  \\ [-\arrayrulewidth]
\cellcolor{colorloc} & OLM &  \conftitle{TIP} & 2020 & Pattern Mining/Transact. & Data mining/CNN layers & pretrained & x  \\ [-\arrayrulewidth]

\rowcolor{rowbackground}
\cellcolor{colorloc} & LOD &  \conftitle{NIPS} & 2021 & Ranking/Graph-based & Quadratic op./PageRank & pretrained & x \\ [-\arrayrulewidth]
\cellcolor{colorloc} & LOST &  \conftitle{BMVC} & 2021 &  &  & pretrained & x \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorloc} & PatchNet &  \conftitle{ARXIV} & 2021 & VAE/Pattern Space & Backprop/Clustering & learned & contrastive   \\ [-\arrayrulewidth]
\cellcolor{colorloc} & TokenCut &  \conftitle{CVPR} & 2022 & Graph-based Spectral & Normalized cut & pretrained & x  \\ [-\arrayrulewidth]



\rowcolor{rowbackground}
\multirow[c]{-14}{0.7em}{\cellcolor{colorloc}
\begin{sideways}\textcolor{white}{\textbf{LOCALIZATION}}\end{sideways}} & MOST &  \conftitle{ICCV} & 2023 & Token Clust./Fractal-Based  & Box-counting/Clustering & pretrained & x   \\ [-\arrayrulewidth]

%% ----------------------------------------------------------------------------------------%%
%% --                                  SEGMENTATION                                      --%%
%% ----------------------------------------------------------------------------------------%%
\midrule

\cellcolor{colorseg} & DC & \conftitle{ICML} & 2010 & Semidefinite program & Low-rank op. & Hand-crafted & x \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & CoSand	& \conftitle{ICCV} & 2011 & Temperature maximization & Submodular op.+Ncut & Hand-crafted & x  \\	 [-\arrayrulewidth] 

\cellcolor{colorseg} & IFBM & \conftitle{CVPR} & 2012 & MRF-based & Graph cuts & Hand-crafted & x \\  [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & MCC	& \conftitle{CVPR} & 2012 & Combinatorial pixel labeling & Block-coord. descent & Hand-crafted & x \\  [-\arrayrulewidth] 

\cellcolor{colorseg} & COMP & \conftitle{ICCV} & 2013 & Score-based refinement & Heuristic seg.+Grabcut & Hand-crafted & x \\  [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & CST & \conftitle{ICCV} & 2013 & MRF-based & Graph cuts & Hand-crafted & x \\  [-\arrayrulewidth] 

\cellcolor{colorseg} & HS	& \conftitle{CVPR} & 2013 & Tree-structure graphical & Belief propagation & Hand-crafted & x \\  [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & OD	& \conftitle{CVPR} & 2013 & Pixel correspondence optim. & Coordinate descent & Hand-crafted & x \\ [-\arrayrulewidth]

\cellcolor{colorseg} & GMS	& \conftitle{ICIP} & 2014 & Global saliency fusion & Grabcut & Hand-crafted & x	 \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & CS-ECEM	& \conftitle{TCSVT} & 2014 & Superpixel labelling & \(\alpha\)-Expansion algorithm & Hand-crafted & x \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & SMD	& \conftitle{TPAMI} & 2017 & Structured matrix decomp. & Felzenszwalb algorithm & Hand-crafted & x \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & wCTR & \conftitle{CVPR} & 2014 & Graph-based approach & Least-square op. & Hand-crafted & x \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & DMFC & \conftitle{CVIU} & 2015 & Graph-based approach & Alternating op./Grabcut & Hand-crafted & x \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & MRW & \conftitle{CVPR} & 2015 & Graph-based approach & Random walkers & Hand-crafted & x \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & WSC & \conftitle{CVPR} & 2015 & Dictionary-based saliency & Sparse coding & Hand-crafted & x \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & SCF & \conftitle{TMM} & 2016 & Quadratic programming & Grabcut & Hand-crafted & x \\

\cellcolor{colorseg} & SBF & \conftitle{ICCV} & 2017 & Saliency network & Backprop & Learned & Fused weak saliency \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & NPG & \conftitle{TIP} & 2017 & Mixed-Integer Programs & Grabcut & Learned & x \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & SGC3 & \conftitle{AAAI} & 2017 & Constrained clustering & K-means like optim. & Hand-crafted & x \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & CoAttCNN & \conftitle{IJCA} & 2018 & Two-stage optimization & Backprop & Pretrained & Off-the-shelf proposals \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & CS-GSIN & \conftitle{NEUCOM} & 2018 & Tree structure graph & Grabcut & Hand-crafted & x \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & DFF & \conftitle{ECCV} & 2018 & Non-negative Factorization & Low-rank approx. & Pretrained & x \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & USDNL & \conftitle{CVPR} & 2018 & Saliency network & Backprop & Learned & Off-the-shelf saliency \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & CP-GAN & \conftitle{ARXIV} & 2019 & GAN & Backprop & Learned & Adversarial \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & DeepCO3 & \conftitle{CVPR} & 2019 & Multi-loss optimization & Backprop & Refined \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & IIC & \conftitle{ICCV} & 2019 & Clustering neural network & Backprop & Learned & Mutual inform. \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & ReDo & \conftitle{NIPS} & 2019 & GAN & Backprop & Learned & Aversarial \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & DeepUSPS & \conftitle{NIPS} & 2019 & Saliency network & Backprop & Learned & Pseudo-labels \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & UnsupOD & \conftitle{SYMM.} & 2020 & Segmentation network & Backprop & Learned & Img. reconstruction \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & CS-OHS & \conftitle{JCS} & 2021 & MRF-based & Particle Swarm & Hand-crafted & x \\	 [-\arrayrulewidth] 

\cellcolor{colorseg} & DRC & \conftitle{NIPS} & 2021 & Generative modeling - MoE & EM-like/MCMC/Bprop & Learned & Img. reconstruction \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & E-BigBigGAN & \conftitle{PMLR} & 2021 & Segmentation network & Backprop & Refined & Synthetic masks \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & MaskContrast & \conftitle{ICCV} & 2021 & Pixel-embedding learning & Backprop & Learned & Contrastive \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & PiCIE & \conftitle{CVPR} & 2021 & Pixel-embedding learning & Backprop & Refined & Cluster assignments \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & UVISAM & \conftitle{BMVC} & 2022 & Segmentation network & Backprop & Refined \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & DSM & \conftitle{CVPR} & 2022 & Graph-based Spectral & Normalized cut & Pretrained & x \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & MOVE & \conftitle{NIPS} & 2022 & Segmenter/inpainter net. & Bprop/Adversarial tr. & Pretrained & composite image \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & SegDiscover & \conftitle{ARXIV} & 2022 & Segmentation network & Backprop & Refined & Cluster assignments \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & SegSwap & \conftitle{CVPR} & 2022 & Graph-based Pair Matching & Grabcut & Pretrained & Correspondence pairs \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & SelfMask & \conftitle{CVPRw} & 2022 & Saliency network & Backprop & Learned & Ranked saliency mask \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & TokenCut & \conftitle{CVPR} & 2022 & Graph-based Spectral & Normalized cut & Pretrained & x \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & CutLER & \conftitle{CVPR} & 2023 & Segmentation network & Ncut/Backprop & Pretrained & MaskCut pseudo-labels \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & SEMPART & \conftitle{ICCV} & 2023 & Graph-based approach & Backprop & Refined & Coarse/fine bi-partition \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}

\multirow[c]{-44}{0.7em}{\cellcolor{colorseg}
\begin{sideways}\textcolor{white}{\textbf{SEGMENTATION}}\end{sideways}} & 
U2Seg & \conftitle{CVPR} & 2024 & Segmentation network & EM/Backprop & Refined & Pseudo-labels \\ [-\arrayrulewidth] 


%% ----------------------------------------------------------------------------------------%%
%% --                                  DECOMPOSITION                                     --%%
%% ----------------------------------------------------------------------------------------%%
\midrule

\cellcolor{colordec} & AIR	& \conftitle{NIPS} & 2016 & VAE	& Variational Bayes & Learned & ELBO	\\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colordec} & CST-VAE	& \conftitle{ICLR} 	& 2016	& VAE	& Variational Bayes & Learned & ELBO	\\ [-\arrayrulewidth] 
\cellcolor{colordec} & TAGGER & \conftitle{NIPS} & 2016 & Denoising AE & Backprop & Learned & NLL \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colordec} & N-EM & \conftitle{NIPS} & 2017 & Recurrent AE & Backprop & Learned & Clustering \\ [-\arrayrulewidth] 
\cellcolor{colordec} & R-NEM & \conftitle{ICLR} & 2018 & Recurrent AE & Backprop & Learned & Clustering \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colordec} & SQAIR & \conftitle{NIPS} & 2018 & Recurrent VAE & Variational Bayes & Learned & IWAE \\ [-\arrayrulewidth] 
\cellcolor{colordec} & GMIO & \conftitle{ICML} & 2019 & Encoder/Decoder &  & Learned & ELBO \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colordec} & IODINE & \conftitle{ICML} & 2019 & VAE & Variational Bayes/IAI & Learned & weigthed ELBO \\ [-\arrayrulewidth] 
\cellcolor{colordec} & MONet & \conftitle{ARXIV} & 2019 & Recurrent VAE & Variational Bayes & Learned & ELBO+KL term \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colordec} & SCAE & \conftitle{NIPS} & 2019 & Capsule Autoencoder  & Backprop & Learned & Log-likelihood \\ [-\arrayrulewidth] 
\cellcolor{colordec} & SPAIR & \conftitle{AAAI} & 2019 & VAE & Variational Bayes & Learned & ELBO \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colordec} & SuPAIR & \conftitle{ICML} & 2019 & Sum-product Network &  & Learned & ELBO \\ [-\arrayrulewidth] 
\cellcolor{colordec} & ECON  & \conftitle{ICLR} & 2020 & Encoder/Decoder &  & Learned & ELBO \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colordec} & GENESIS & \conftitle{ICLR} & 2020 & Encoder/Decoder &  & Learned & GECO \\ [-\arrayrulewidth] 
\cellcolor{colordec} & GNM & \conftitle{NIPS} & 2020 & Encoder/Decoder &  & Learned & ELBO \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colordec} & LMIO & \conftitle{CVPR} & 2020 & Encoder/Decoder &  & Learned & IBL \\ [-\arrayrulewidth] 
\cellcolor{colordec} & MulMON & \conftitle{NIPS} & 2020 & Encoder/Decoder &  & Learned & ELBO \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colordec} & SCALOR & \conftitle{ICLR} & 2020 & Encoder/Decoder &  & Learned & ELBO \\  [-\arrayrulewidth] 
\cellcolor{colordec} & SLOT ATTENTION & \conftitle{NIPS} & 2020 & Differentiable interface &  & Refined & x \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colordec} & SPACE & \conftitle{ICLR} & 2020 & Encoder/Decoder &  & Learned & ELBO\\ [-\arrayrulewidth] 
\cellcolor{colordec} & SRN & \conftitle{NIPS} & 2020 & Differentiable interface &  & Refined & x \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colordec} & DTISprites & \conftitle{ICCV} & 2021 & Transform Predictor &  & Learned & Reconstruction $L_2$ \\ [-\arrayrulewidth] 
\cellcolor{colordec} & EfficientMORL & \conftitle{ICML} & 2021 & Encoder/Decoder &  & Learned & weigthed ELBO \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colordec} & GENESISv2 & \conftitle{NIPS} & 2021 & Encoder/Decoder &  & Learned & GECO \\ [-\arrayrulewidth] 
\cellcolor{colordec} & GMAIR & \conftitle{CIN} & 2021 & Encoder/Decoder &  & Learned & ELBO \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colordec} & GSNGs & \conftitle{ICLR} & 2021 & Encoder/Decoder &  & Learned & ELBO \\ [-\arrayrulewidth] 
\cellcolor{colordec} & MarioNette & \conftitle{NIPS} & 2021 & Transform Predictor &  & Learned & Reconstruction $L_2$ \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colordec} & uORF & \conftitle{ICLR} & 2022 & Encoder/Decoder &  & Learned & Reconstruction $L_2$ \\ [-\arrayrulewidth] 

\multirow[c]{-29}{0.7em}{\cellcolor{colordec}
\begin{sideways}\textcolor{white}{\textbf{DECOMPOSITION}}\end{sideways}} & 
DINOSAUR & \conftitle{ICLR} & 2023 & Encoder/Decoder & Backprop/Slot Attn. & Refined & Reconstruction $L_2$ \\ [-\arrayrulewidth] 


 \bottomrule

\end{tabular}%
}
\caption{Overview of shared characteristics of methods across the four different groups in Unsupervised Object Discovery.}
\label{tab:overview_dec}
\end{longtable}

==> tables/table_overview_all_prop.tex <==
\let\conftitle\tiny


%\begin{longtable}[]
{\tiny\tabcolsep=4pt  
%\footnotesize

\captionsetup[longtable]{width=0.93\linewidth} 
\captionsetup[longtable]{skip=2.5em}
\begin{longtable}{p{0.7em}lccccccccc}


%\setlength{\aboverulesep}{0pt} % Reduce space above rules
%\setlength{\belowrulesep}{0pt} % Reduce space below rules
%\begin{tabular}{clcccccc}
%>{\kern-\tabcolsep}
%\begin{tabular}{@{}clcccccc@{}}
%\toprule
\toprule
%\specialrule{*}{0pt}{0pt}
\multicolumn{11}{c}{\cellcolor[HTML]{DDDDDD} {\MakeUppercase{properties among Methods in this survey}}}                                 \\ \midrule
   &
  Method &
  \begin{tabular}[c]{@{}c@{}}Pub.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Year\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Intra-image \\ Similarities\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Inter-image \\ Similarities\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Probabilistic \\ formulations\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Graph-based \\ techniques\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Generative \\ modeling\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Deep \\ learning\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Code \\ released\end{tabular} \\ \midrule


\endfirsthead


\multicolumn{11}{c}{\cellcolor[HTML]{DDDDDD} {\MakeUppercase{properties among Methods in this survey}}}                                \\ \midrule
   &
  Method &
  \begin{tabular}[c]{@{}c@{}}Pub.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Year\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Intra-image \\ Similarities\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Inter-image \\ Similarities\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Probabilistic \\ formulations\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Graph-based \\ techniques\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Generative \\ modeling\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Deep \\ learning\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Code \\ released\end{tabular} \\ \midrule


\endhead            
\midrule\multicolumn{11}{c}{{Continued on next page}} \\ \midrule
\endfoot    
%\bottomrule     
\endlastfoot






%% ----------------------------------------------------------------------------------------%%
%% --                                  CLUSTERING                                        --%%
%% ----------------------------------------------------------------------------------------%%

\cellcolor{colorclust}& DEC & \conftitle{ICML} & 2015 & \EMPTY & \EMPTY & \CHECK & \EMPTY & \EMPTY & \CHECK & \CHECK  \\ [-\arrayrulewidth]

\rowcolor{rowbackground}
 \cellcolor{colorclust}& AAE	& \conftitle{ARXIV} & 2016 & \EMPTY & \EMPTY & \CHECK & \EMPTY & \CHECK & \CHECK & \EMPTY  \\ [-\arrayrulewidth]
\cellcolor{colorclust}& JULE & \conftitle{CVPR} & 2016 & \EMPTY & \CHECK & \EMPTY & \CHECK & \EMPTY & \CHECK & \CHECK  \\ [-\arrayrulewidth]

\rowcolor{rowbackground}
\cellcolor{colorclust} & DAC & \conftitle{ICCV} & 2017 & \EMPTY & \CHECK & \EMPTY & \EMPTY & \EMPTY & \CHECK & \CHECK  \\ [-\arrayrulewidth]
\cellcolor{colorclust} & GMVAE & \conftitle{ICLR} & 2017 & \EMPTY & \EMPTY & \CHECK & \EMPTY & \CHECK & \CHECK & \CHECK  \\ [-\arrayrulewidth]

\rowcolor{rowbackground}
\cellcolor{colorclust} & IMSAT & \conftitle{ICML} & 2017 & \CHECK & \EMPTY & \CHECK & \EMPTY & \EMPTY & \CHECK & \CHECK  \\ [-\arrayrulewidth]
\cellcolor{colorclust} & ADC	& \conftitle{GCPR} & 2018 & \CHECK & \EMPTY & \CHECK & \EMPTY & \EMPTY & \CHECK & \EMPTY  \\ [-\arrayrulewidth]

\rowcolor{rowbackground}
\cellcolor{colorclust} & FineGAN & \conftitle{CVPR} & 2019 & \CHECK & \EMPTY & \CHECK & \EMPTY & \CHECK & \CHECK & \CHECK  \\ [-\arrayrulewidth]
\cellcolor{colorclust} & IIC & \conftitle{ICCV} & 2019 & \CHECK & \EMPTY & \CHECK & \EMPTY & \EMPTY & \CHECK & \CHECK  \\ [-\arrayrulewidth]

\rowcolor{rowbackground}
\cellcolor{colorclust} & DTI-GMM	& \conftitle{NIPS} & 2020 & \CHECK & \EMPTY & \CHECK & \EMPTY & \EMPTY & \CHECK & \CHECK  \\ [-\arrayrulewidth]
\cellcolor{colorclust} & SCAN & \conftitle{ECCV} & 2020 & \CHECK & \CHECK & \EMPTY & \EMPTY & \EMPTY & \CHECK & \CHECK \\ [-\arrayrulewidth]

\rowcolor{rowbackground}
\multirow[c]{-12}{0.7em}{\cellcolor{colorclust}
\begin{sideways}\textcolor{white}{\textbf{CLUSTERING}}\end{sideways}} & TwoFoldOp & \conftitle{NEUROC} & 2022 & \CHECK & \CHECK & \CHECK & \EMPTY & \EMPTY & \CHECK & \EMPTY  \\ [-\arrayrulewidth]

%% ----------------------------------------------------------------------------------------%%
%% --                                  LOCALIZATION                                      --%%
%% ----------------------------------------------------------------------------------------%%
\midrule

\cellcolor{colorloc} & CL-FWA &  \conftitle{ECCV} & 2014 & \CHECK & \CHECK & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \EMPTY \\ [-\arrayrulewidth]

\rowcolor{rowbackground}
\cellcolor{colorloc} & CL-CSD &  \conftitle{ECCV} & 2016 & \EMPTY & \EMPTY & \CHECK & \CHECK & \EMPTY & \EMPTY & \EMPTY  \\ [-\arrayrulewidth]
\cellcolor{colorloc} & OLM &  \conftitle{TIP} & 2020 & \CHECK & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \EMPTY  \\ [-\arrayrulewidth]

\rowcolor{rowbackground}
\cellcolor{colorloc} & LOD &  \conftitle{NIPS} & 2021 & \EMPTY & \EMPTY & \EMPTY & \CHECK & \EMPTY & \EMPTY & \CHECK \\ [-\arrayrulewidth]
\cellcolor{colorloc} & LOST &  \conftitle{BMVC} & 2021 & \CHECK & \EMPTY & \EMPTY & \CHECK & \EMPTY & \EMPTY & \CHECK \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorloc} & PatchNet &  \conftitle{ARXIV} & 2021 & \CHECK & \CHECK & \CHECK & \EMPTY & \CHECK & \CHECK & \EMPTY   \\ [-\arrayrulewidth]
\cellcolor{colorloc} & TokenCut &  \conftitle{CVPR} & 2022 & \CHECK & \EMPTY & \EMPTY & \CHECK & \EMPTY & \CHECK & \CHECK  \\ [-\arrayrulewidth]

\rowcolor{rowbackground}
\cellcolor{colorloc} & MOST &  \conftitle{ICCV} & 2023 & \CHECK & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \CHECK & \CHECK  \\ [-\arrayrulewidth]
\cellcolor{colorloc} & OLM &  \conftitle{TIP} & 2020 & \CHECK & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \EMPTY  \\ [-\arrayrulewidth]

\rowcolor{rowbackground}
\cellcolor{colorloc} & LOD &  \conftitle{NIPS} & 2021 & \EMPTY & \EMPTY & \EMPTY & y & \EMPTY & \EMPTY & \CHECK \\ [-\arrayrulewidth]
\cellcolor{colorloc} & LOST &  \conftitle{BMVC} & 2021 & \CHECK & \EMPTY & \EMPTY & \CHECK & \EMPTY & \EMPTY & \CHECK \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorloc} & PatchNet &  \conftitle{ARXIV} & 2021 & \CHECK & \CHECK & \CHECK & \EMPTY & \CHECK & \CHECK & \EMPTY   \\ [-\arrayrulewidth]
\cellcolor{colorloc} & TokenCut &  \conftitle{CVPR} & 2022 & \CHECK & \EMPTY & \EMPTY & \CHECK & \EMPTY & \CHECK & \CHECK  \\ [-\arrayrulewidth]



\rowcolor{rowbackground}
\multirow[c]{-14}{0.7em}{\cellcolor{colorloc}
\begin{sideways}\textcolor{white}{\textbf{LOCALIZATION}}\end{sideways}} & MOST &  \conftitle{ICCV} & 2023 & \CHECK & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \CHECK & \CHECK   \\ [-\arrayrulewidth]

%% ----------------------------------------------------------------------------------------%%
%% --                                  SEGMENTATION                                      --%%
%% ----------------------------------------------------------------------------------------%%

\midrule

\cellcolor{colorseg} & DC & \conftitle{ICML} & 2010 & \CHECK & \CHECK & \EMPTY & \CHECK & \EMPTY & \EMPTY & \CHECK \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & CoSand	& \conftitle{ICCV} & 2011 & \CHECK & \CHECK & \EMPTY & \CHECK & \EMPTY & \EMPTY & \CHECK  \\	 [-\arrayrulewidth] 

\cellcolor{colorseg} & IFBM & \conftitle{CVPR} & 2012 & \CHECK & \CHECK & \CHECK & \CHECK & \CHECK & \EMPTY & \EMPTY \\  [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & MCC	& \conftitle{CVPR} & 2012 & \CHECK & \CHECK & \CHECK & \CHECK & \EMPTY & \EMPTY & \CHECK \\  [-\arrayrulewidth] 

\cellcolor{colorseg} & COMP & \conftitle{ICCV} & 2013 & \CHECK & \CHECK & \CHECK & \CHECK & \EMPTY & \EMPTY & \CHECK \\  [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & CST & \conftitle{ICCV} & 2013 & \CHECK & \CHECK & \CHECK & \CHECK & \EMPTY & \EMPTY & \CHECK \\  [-\arrayrulewidth] 

\cellcolor{colorseg} & HS	& \conftitle{CVPR} & 2013 & \CHECK & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \EMPTY \\  [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & OD	& \conftitle{CVPR} & 2013 & \CHECK & \CHECK & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \CHECK \\ [-\arrayrulewidth]

\cellcolor{colorseg} & GMS	& \conftitle{ICIP} & 2014 & \CHECK & \CHECK & \EMPTY & \CHECK & \EMPTY & \EMPTY & \CHECK	 \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & CS-ECEM	& \conftitle{TCSVT} & 2014 & \CHECK & \CHECK & \EMPTY & \CHECK & \EMPTY & \EMPTY & \EMPTY \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & wCTR & \conftitle{CVPR} & 2014 & \CHECK & \EMPTY & \EMPTY & \CHECK & \EMPTY & \EMPTY & \CHECK \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & DMFC & \conftitle{CVIU} & 2015 & \CHECK & \CHECK & \CHECK & \CHECK & \EMPTY & \EMPTY & \CHECK \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & MRW & \conftitle{CVPR} & 2015 & \CHECK & \CHECK & \CHECK & \CHECK & \EMPTY & \EMPTY & \EMPTY \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & WSC & \conftitle{CVPR} & 2015 & \CHECK & \EMPTY & \EMPTY & \CHECK & \EMPTY & \EMPTY & \CHECK \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & SCF & \conftitle{TMM} & 2016 & \EMPTY & \CHECK & \EMPTY & \CHECK & \EMPTY & \EMPTY & \CHECK \\

\rowcolor{rowbackground}
\cellcolor{colorseg} & SMD	& \conftitle{TPAMI} & 2016 & \CHECK & \EMPTY & \EMPTY & \CHECK & \EMPTY & \EMPTY & \EMPTY \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & NPG & \conftitle{TIP} & 2017 & \EMPTY & \CHECK & \CHECK & \CHECK & \EMPTY & \CHECK & \EMPTY \\ [-\arrayrulewidth] 


\rowcolor{rowbackground}
\cellcolor{colorseg} & SBF & \conftitle{ICCV} & 2017 & \EMPTY & \EMPTY & \CHECK & \EMPTY & \EMPTY & \CHECK & \CHECK \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & SGC3 & \conftitle{AAAI} & 2017 & \EMPTY & \CHECK & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \EMPTY \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & CoAttCNN & \conftitle{IJCA} & 2018 & \EMPTY & \CHECK & \EMPTY & \EMPTY & \EMPTY & \CHECK & \EMPTY \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & CS-GSIN & \conftitle{NEUCOM} & 2018 & \CHECK & \CHECK & \EMPTY & \CHECK & \EMPTY & \EMPTY & \EMPTY \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & DFF & \conftitle{ECCV} & 2018 & \EMPTY & \CHECK & \EMPTY & \EMPTY & \EMPTY & \CHECK & \CHECK \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & USDNL & \conftitle{CVPR} & 2018 & \EMPTY & \EMPTY & \CHECK & \EMPTY & \EMPTY & \CHECK & \EMPTY \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & CP-GAN & \conftitle{ARXIV} & 2019 & \EMPTY & \EMPTY & \CHECK & \EMPTY & \CHECK & \CHECK & \EMPTY \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & DeepCO3 & \conftitle{CVPR} & 2019 & \EMPTY & \CHECK & \EMPTY & \EMPTY & \EMPTY & \CHECK & \CHECK \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & IIC & \conftitle{ICCV} & 2019 & \CHECK & \EMPTY & \CHECK & \EMPTY & \EMPTY & \CHECK & \CHECK \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & ReDo & \conftitle{NIPS} & 2019 & \EMPTY & \EMPTY & \CHECK & \EMPTY & \CHECK & \CHECK & \EMPTY \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & DeepUSPS & \conftitle{NIPS} & 2019 & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \CHECK & \CHECK \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & UnsupOD & \conftitle{SYMM.} & 2020 & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \CHECK & \EMPTY \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & CS-OHS & \conftitle{JCS} & 2021 & \EMPTY & \CHECK & \EMPTY & \EMPTY & \EMPTY & \CHECK & \EMPTY \\	 [-\arrayrulewidth] 

\cellcolor{colorseg} & DRC & \conftitle{NIPS} & 2021 & \EMPTY & \EMPTY & \CHECK & \EMPTY & \CHECK & \CHECK & \CHECK \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & E-BigBigGAN & \conftitle{PMLR} & 2021 & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \CHECK & \CHECK \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & MaskContrast & \conftitle{ICCV} & 2021 & \CHECK & \CHECK & \EMPTY & \EMPTY & \EMPTY & \CHECK & \CHECK \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & PiCIE & \conftitle{CVPR} & 2021 & \EMPTY & \CHECK & \EMPTY & \EMPTY & \EMPTY & \CHECK & \CHECK \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & UVISAM & \conftitle{BMVC} & 2022 & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \CHECK & \CHECK \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & DSM & \conftitle{CVPR} & 2022 & \CHECK & \CHECK & \EMPTY & \CHECK & \EMPTY & \CHECK & \CHECK \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & MOVE & \conftitle{NIPS} & 2022 & \CHECK & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \CHECK & \CHECK \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & SegDiscover & \conftitle{ARXIV} & 2022 & \EMPTY & \CHECK & \EMPTY & \EMPTY & \EMPTY & \CHECK & \EMPTY \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & SegSwap & \conftitle{CVPR} & 2022 & \EMPTY & \CHECK & \EMPTY & \CHECK & \EMPTY & \CHECK & \CHECK \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & SelfMask & \conftitle{CVPRw} & 2022 & \CHECK & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \CHECK & \CHECK \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & TokenCut & \conftitle{CVPR} & 2022 & \CHECK & \EMPTY & \EMPTY & \CHECK & \EMPTY & \CHECK & \CHECK \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colorseg} & CutLER & \conftitle{CVPR} & 2023 & \CHECK & \EMPTY & \EMPTY & \CHECK & \EMPTY & \CHECK & \CHECK \\ [-\arrayrulewidth] 

\cellcolor{colorseg} & SEMPART & \conftitle{ICCV} & 2023 & \CHECK & \EMPTY & \EMPTY & \CHECK & \EMPTY & \CHECK & \EMPTY \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}

\multirow[c]{-44}{0.7em}{\cellcolor{colorseg}
\begin{sideways}\textcolor{white}{\textbf{SEGMENTATION}}\end{sideways}} & 
U2Seg & \conftitle{CVPR} & 2024 & \CHECK & \CHECK & \EMPTY & \EMPTY & \EMPTY & \CHECK & \CHECK \\ [-\arrayrulewidth] 


%% ----------------------------------------------------------------------------------------%%
%% --                                  DECOMPOSITION                                     --%%
%% ----------------------------------------------------------------------------------------%%
\midrule

\cellcolor{colordec} & AIR	& \conftitle{NIPS} & 2016 & \EMPTY & \EMPTY & \CHECK & \EMPTY & \CHECK & \CHECK & \CHECK	\\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colordec} & CST-VAE	& \conftitle{ICLR} 	& 2016	& \EMPTY & \EMPTY & \CHECK & \EMPTY & \CHECK & \CHECK & \EMPTY	\\ [-\arrayrulewidth] 
\cellcolor{colordec} & TAGGER & \conftitle{NIPS} & 2016 & ? & ? & \CHECK & ? & ? & ? & \CHECK \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colordec} & N-EM & \conftitle{NIPS} & 2017 & ? & ? & \CHECK & ? & ? & ? & \CHECK \\ [-\arrayrulewidth] 
\cellcolor{colordec} & R-NEM & \conftitle{ICLR} & 2018 & ? & ? & \CHECK & ? & ? & ? & \CHECK \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colordec} & SQAIR & \conftitle{NIPS} & 2018 & ? & ? & \CHECK & ? & ? & ? & \CHECK \\ [-\arrayrulewidth] 
\cellcolor{colordec} & GMIO & \conftitle{ICML} & 2019 & ? & ? & \CHECK & ? & ? & ? & \EMPTY \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colordec} & IODINE & \conftitle{ICML} & 2019 & ? & ? & \CHECK & ? & ? & ? & \CHECK \\ [-\arrayrulewidth] 
\cellcolor{colordec} & MONet & \conftitle{ARXIV} & 2019 & ? & ? & \CHECK & ? & ? & ? & \EMPTY \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colordec} & SCAE & \conftitle{NIPS} & 2019 & ? & ? & \EMPTY & ? & ? & ? & \CHECK \\ [-\arrayrulewidth] 
\cellcolor{colordec} & SPAIR & \conftitle{AAAI} & 2019 & ? & ? & \CHECK & ? & ? & ? & \CHECK \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colordec} & SuPAIR & \conftitle{ICML} & 2019 & ? & ? & \CHECK & ? & ? & ? & \CHECK \\ [-\arrayrulewidth] 
\cellcolor{colordec} & ECON  & \conftitle{ICLR} & 2020 & ? & ? & \CHECK & ? & ? & ? & \EMPTY \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colordec} & GENESIS & \conftitle{ICLR} & 2020 & ? & ? & \CHECK & ? & ? & ? & \CHECK \\ [-\arrayrulewidth] 
\cellcolor{colordec} & GNM & \conftitle{NIPS} & 2020 & ? & ? & \CHECK & ? & ? & ? & \CHECK \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colordec} & LMIO & \conftitle{CVPR} & 2020 & ? & ? & \CHECK & ? & ? & ? & \CHECK \\ [-\arrayrulewidth] 
\cellcolor{colordec} & MulMON & \conftitle{NIPS} & 2020 & ? & ? & \CHECK & ? & ? & ? & \CHECK \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colordec} & SCALOR & \conftitle{ICLR} & 2020 & ? & ? & \CHECK & ? & ? & ? & \CHECK \\  [-\arrayrulewidth] 
\cellcolor{colordec} & SLOT ATTN. & \conftitle{NIPS} & 2020 & ? & ? & \EMPTY & ? & ? & ? & \CHECK \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colordec} & SPACE & \conftitle{ICLR} & 2020 & ? & ? & \CHECK & ? & ? & ? & \CHECK\\ [-\arrayrulewidth] 
\cellcolor{colordec} & SRN & \conftitle{NIPS} & 2020 & ? & ? & \EMPTY & ? & ? & ? & \CHECK \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colordec} & DTISprites & \conftitle{ICCV} & 2021 & ? & ? & \EMPTY & ? & ? & ? & \CHECK \\ [-\arrayrulewidth] 
\cellcolor{colordec} & EfficientMORL & \conftitle{ICML} & 2021 & ? & ? & \CHECK & ? & ? & ? & \CHECK \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colordec} & GENESISv2 & \conftitle{NIPS} & 2021 & ? & ? & \CHECK & ? & ? & ? & \CHECK \\ [-\arrayrulewidth] 
\cellcolor{colordec} & GMAIR & \conftitle{CIN} & 2021 & ? & ? & \CHECK & ? & ? & ? & \CHECK \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colordec} & GSNGs & \conftitle{ICLR} & 2021 & ? & ? & \CHECK & ? & ? & ? & \CHECK \\ [-\arrayrulewidth] 
\cellcolor{colordec} & MarioNette & \conftitle{NIPS} & 2021 & ? & ? & \EMPTY & ? & ? & ? & \CHECK \\ [-\arrayrulewidth] 

\rowcolor{rowbackground}
\cellcolor{colordec} & uORF & \conftitle{ICLR} & 2022 & ? & ? & \EMPTY & ? & ? & ? & \CHECK \\ [-\arrayrulewidth] 

\multirow[c]{-29}{0.7em}{\cellcolor{colordec}
\begin{sideways}\textcolor{white}{\textbf{DECOMPOSITION}}\end{sideways}} & 
DINOSAUR & \conftitle{ICLR} & 2023 & ? & ? & \EMPTY & ? & ? & ? & \CHECK \\ [-\arrayrulewidth] 


 \bottomrule

%\end{tabular}%
\caption{Overview of shared properties of methods across the four different groups in Unsupervised Object Discovery.} 

\label{tab:overview_all_prop}
\end{longtable}
}

==> tables/table_overview_clust.tex <==
\let\conftitle\footnotesize

\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccccccccc@{}}
\toprule
\multicolumn{15}{c}{Clustering Methods}                                 \\ \midrule
Method &
  \begin{tabular}[c]{@{}c@{}}Pub.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Year\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Model \\ Formulation\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Optimization\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Representation\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Learning\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Membership\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Intra-Img\\ Sim.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Inter-Img\\ Sim.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Probabilistic\\ formulation\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Generative\\ Modeling\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Graph-based\\ Techniques\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Deep\\ Learning\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Code\\ Released\end{tabular} \\ \midrule

DEC & \conftitle{ICML} & 2015 & Repr. learning+Probab. clust. & Backprop/Refinement (k-means) & Learned & Target distrib. & T-distrib. kernel & \EMPTY & \EMPTY & \EMPTY & \CHECK & \EMPTY & \CHECK & \CHECK \\

AAE	& \conftitle{ARXIV} & 2016 & Autoencoder + Adversarial Net & Backprop/Adversarial training & Learned & Img. reconstruction & Softmax & \EMPTY & \EMPTY & \CHECK & \CHECK & \EMPTY & \CHECK & \EMPTY \\

JULE & \conftitle{CVPR} & 2016 & Rec. CNN+Agglom. Clust. & Backprop/Greedy Search & Learned & Weighted triplet loss & Cluster labels & \EMPTY & \CHECK & \EMPTY & \EMPTY & \CHECK & \CHECK & \CHECK \\

DAC & \conftitle{ICCV} & 2017 & Binary Pairwise-Classifier & Backprop/Adaptive training & Pretrained & Pairwise similarities & Softmax & \EMPTY & \CHECK & \EMPTY & \EMPTY & \EMPTY & \CHECK & \CHECK \\

GMVAE & \conftitle{ICLR} & 2017 & Variational autoencoder & Backprop/Variational inference & Learned & ELBO & GMM & \EMPTY & \EMPTY & \CHECK & \CHECK & \EMPTY & \CHECK & \CHECK \\

IMSAT & \conftitle{ICML} & 2017 & discrete repr. learning & Backprop/Information Theory & Pretrained & Transformations/MI & Softmax & \CHECK & \EMPTY & \EMPTY & \CHECK & \EMPTY & \CHECK & \CHECK \\

ADC	& \conftitle{GCPR} & 2018 & Classification network & Backprop/Associative clustering & Learned & Transform. invariant loss & Softmax & \CHECK & \EMPTY & \EMPTY & \CHECK & \EMPTY & \CHECK & \EMPTY \\

FineGAN & \conftitle{CVPR} & 2019 & Hierarchical GAN & Backprop/Adversarial training & Learned & Adversarial + MI & K-means & \CHECK & \EMPTY & \CHECK & \CHECK & \EMPTY & \CHECK & \CHECK \\

IIC & \conftitle{ICCV} & 2019 & Classification network & Backprop/Information Theory & Learned & Transformations/MI & Softmax & \CHECK & \EMPTY & \EMPTY & \CHECK & \EMPTY & \CHECK & \CHECK \\

DTI-GMM	& \conftitle{NIPS} & 2020 & Transformation Prediction & Backprop/EM & - & Transform. invariant loss & Closest prot. & \CHECK & \EMPTY & \EMPTY & \CHECK & \EMPTY & \CHECK & \CHECK \\

SCAN & \conftitle{ECCV} & 2020 & Repr. learning+Classif. net. & Backprop/Nearest neighbors & Learned & Semantic clustering loss & Softmax & \CHECK & \CHECK & \EMPTY & \EMPTY & \EMPTY & \CHECK & \CHECK \\

TwoFoldOp & \conftitle{NEUROC} & 2022 & Repr. learning+Classif. net. & Backprop/Alternating loss (EM-like) & Learned & Clust. loss/ KL aug. & Softmax & \CHECK & \CHECK & \EMPTY & \CHECK & \EMPTY & \CHECK & \EMPTY \\




 \bottomrule




\end{tabular}%
}
\caption{Overview of clustering methods and common techniques employed in UOD.}
\label{tab:overview_dec}
\end{table}

==> tables/table_overview_clust_a.tex <==
\let\conftitle\footnotesize

\begin{table}[]
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lccccccc@{}}
\toprule
\multicolumn{8}{c}{\cellcolor{colorclust}{\textcolor{white}{\textbf{Clustering Methods}}}}                                 \\ \midrule
  Method &
  \begin{tabular}[c]{@{}c@{}}Pub.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Year\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Model\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Optimization\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Representation\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Learning\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Membership\end{tabular} \\ \midrule

DEC & \conftitle{ICML} & 2015 & Repr. Learning/Probab. Clust. & Backprop/Refinement (k-means) & Learned & Target distrib. & T-distrib. kernel \\

AAE	& \conftitle{ARXIV} & 2016 & Autoencoder/Adversarial Net & Backprop/Adversarial training & Learned & Img. reconstruction & Softmax \\

JULE & \conftitle{CVPR} & 2016 & Rec. CNN/Agglom. Clust. & Backprop/Greedy Search & Learned & Weighted triplet loss & Cluster labels \\

DAC & \conftitle{ICCV} & 2017 & Binary Pairwise-Classifier & Backprop/Adaptive training & Pretrained & Pairwise similarities & Softmax \\

GMVAE & \conftitle{ICLR} & 2017 & Variational autoencoder & Backprop/Variational inference & Learned & ELBO & GMM \\

IMSAT & \conftitle{ICML} & 2017 & discrete repr. learning & Backprop/Information Theory & Pretrained & Transformations/MI & Softmax \\

ADC	& \conftitle{GCPR} & 2018 & Classification network & Backprop/Associative clustering & Learned & Transform. invariant loss & Softmax \\

FineGAN & \conftitle{CVPR} & 2019 & Hierarchical GAN & Backprop/Adversarial training & Learned & Adversarial + MI & K-means \\

IIC & \conftitle{ICCV} & 2019 & Classification network & Backprop/Information Theory & Learned & Transformations/MI & Softmax \\

DTI-GMM	& \conftitle{NIPS} & 2020 & Transformation Prediction & Backprop/EM & - & Transform. invariant loss & Closest prot. \\

SCAN & \conftitle{ECCV} & 2020 & Repr. learning+Classif. net. & Backprop/Nearest neighbors & Learned & Semantic clustering loss & Softmax \\

TwoFoldOp & \conftitle{NEUROC} & 2022 & Repr. learning+Classif. net. & Backprop/Alternating loss (EM-like) & Learned & Clust. loss/ KL aug. & Softmax \\


 \bottomrule


\end{tabular}%
}
\caption{Overview of clustering methods and common techniques employed in UOD.}
\label{tab:overview_dec}
\end{table}

==> tables/table_overview_clust_b.tex <==
\let\conftitle\footnotesize

\begin{table}[]
\centering
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{@{}lccccccccc@{}}
\toprule
\multicolumn{10}{c}{\cellcolor{colorclust}{\textcolor{white}{\textbf{Clustering Methods}}}}                                 \\ \midrule
  Method &
  \begin{tabular}[c]{@{}c@{}}Pub.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Year\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Intra-Img\\ Sim.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Inter-Img\\ Sim.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Probabilistic\\ formulation\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Generative\\ Modeling\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Graph-based\\ Techniques\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Deep\\ Learning\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Code\\ Released\end{tabular} \\ \midrule

DEC & \conftitle{ICML} & 2015 & \EMPTY & \EMPTY & \EMPTY & \CHECK & \EMPTY & \CHECK & \CHECK \\

AAE	& \conftitle{ARXIV} & 2016 & \EMPTY & \EMPTY & \CHECK & \CHECK & \EMPTY & \CHECK & \EMPTY \\

JULE & \conftitle{CVPR} & 2016 & \EMPTY & \CHECK & \EMPTY & \EMPTY & \CHECK & \CHECK & \CHECK \\

DAC & \conftitle{ICCV} & 2017 & \EMPTY & \CHECK & \EMPTY & \EMPTY & \EMPTY & \CHECK & \CHECK \\

GMVAE & \conftitle{ICLR} & 2017 & \EMPTY & \EMPTY & \CHECK & \CHECK & \EMPTY & \CHECK & \CHECK \\

IMSAT & \conftitle{ICML} & 2017 & \CHECK & \EMPTY & \EMPTY & \CHECK & \EMPTY & \CHECK & \CHECK \\

ADC	& \conftitle{GCPR} & 2018 & \CHECK & \EMPTY & \EMPTY & \CHECK & \EMPTY & \CHECK & \EMPTY \\

FineGAN & \conftitle{CVPR} & 2019 & \CHECK & \CHECK & \EMPTY & \CHECK & \CHECK \\

IIC & \conftitle{ICCV} & 2019 & \CHECK & \EMPTY & \EMPTY & \CHECK & \EMPTY & \CHECK & \CHECK \\

DTI-GMM	& \conftitle{NIPS} & 2020 & \CHECK & \EMPTY & \EMPTY & \CHECK & \EMPTY & \CHECK & \CHECK \\

SCAN & \conftitle{ECCV} & 2020 & \CHECK & \CHECK & \EMPTY & \EMPTY & \EMPTY & \CHECK & \CHECK \\

TwoFoldOp & \conftitle{NEUROC} & 2022 & \CHECK & \CHECK & \EMPTY & \CHECK & \EMPTY & \CHECK & \EMPTY \\


 \bottomrule




\end{tabular}%
}
\caption{Overview of clustering methods and common techniques employed in UOD.}
\label{tab:overview_dec}
\end{table}

==> tables/table_overview_dec.tex <==
\let\conftitle\footnotesize

\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lccccccccc@{}}
\toprule
\multicolumn{10}{c}{Decomposition Methods}                                 \\ \midrule
Method &
  \begin{tabular}[c]{@{}c@{}}Published \\ at\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Year\\ available\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Architectural \\ style\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Attention\\ strategy\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Obj. Representation \\ Inference\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Main Training\\ objective\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Additional \\ objectives\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Probabilistic\\ formulation\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Code\\ available\end{tabular} \\ \midrule
AIR & \conftitle{NIPS} & 2016 & Encoder/Decoder & Glimpse-based & Sequential & ELBO & \EMPTY & \CHECK & \CHECK \\
CST-VAE & \conftitle{ICLR} & 2016 & Encoder/Decoder & Glimpse-based & Sequential & ELBO & \EMPTY & \CHECK & \EMPTY \\
TAGGER & \conftitle{NIPS} & 2016 & Encoder/Decoder & Mask-based & Iterative & NLL & \EMPTY & \CHECK & \CHECK \\
N-EM & \conftitle{NIPS} & 2017 & Encoder/Decoder & Mask-based & Iterative & Clustering & \EMPTY & \CHECK & \CHECK \\
R-NEM & \conftitle{ICLR} & 2018 & Encoder/Decoder & Mask-based & Iterative & Clustering & \EMPTY & \CHECK & \CHECK \\
SQAIR & \conftitle{NIPS} & 2018 & Encoder/Decoder & Glimpse-based & Sequential & IWAE & \EMPTY & \CHECK & \CHECK \\
GMIO & \conftitle{ICML} & 2019 & Encoder/Decoder & Glimpse-based & Sequential & ELBO & \EMPTY & \CHECK & \EMPTY \\
IODINE & \conftitle{ICML} & 2019 & Encoder/Decoder & Mask-based & Iterative & weighted ELBO & \EMPTY & \CHECK & \CHECK \\
MONet & arxiv & 2019 & Encoder/Decoder & Mask-based & Sequential & ELBO & \CHECK & \CHECK & \EMPTY \\
SCAE & \conftitle{NIPS} & 2019 & Capsule Autoencoder & \EMPTY & \EMPTY & Log-likelihood & \EMPTY & \EMPTY & \CHECK \\
SPAIR & \conftitle{AAAI} & 2019 & Encoder/Decoder & Glimpse-based & Sequential & ELBO & \EMPTY & \CHECK & \CHECK \\
SuPAIR & \conftitle{ICML} & 2019 & Sum-product Network & Glimpse-based & Sequential & ELBO & \EMPTY & \CHECK & \CHECK \\
ECON & \conftitle{ICLR} & 2020 & Encoder/Decoder & Mask-based & Sequential & ELBO & \EMPTY & \CHECK & \EMPTY \\
GENESIS & \conftitle{ICLR} & 2020 & Encoder/Decoder & Mask-based & Sequential & GECO & \CHECK & \CHECK & \CHECK \\
GNM & \conftitle{NIPS} & 2020 & Encoder/Decoder & Glimpse-based & Sequential & ELBO & \EMPTY & \CHECK & \CHECK \\
LMIO & \conftitle{CVPR} & 2020 & Encoder/Decoder & Mask-based & Sequential & IBL & \CHECK & \CHECK & \CHECK \\
MulMON & \conftitle{NIPS} & 2020 & Encoder/Decoder & Mask-based & Iterative & ELBO & \CHECK & \CHECK & \CHECK \\
SCALOR & \conftitle{ICLR} & 2020 & Encoder/Decoder & Glimpse-based & Sequential & ELBO & \EMPTY & \CHECK & \CHECK \\
SLOT ATTENTION & \conftitle{NIPS} & 2020 & Differentiable interface & Mask-based & Iterative & \EMPTY  & \EMPTY & \EMPTY & \CHECK \\
SPACE & \conftitle{ICLR} & 2020 & Encoder/Decoder & Glimpse-based & Sequential & ELBO & \EMPTY & \CHECK & \CHECK \\
SRN & \conftitle{NIPS} & 2020 & Differentiable interface & Mask-based & Iterative & \EMPTY  & \EMPTY & \EMPTY & \CHECK \\
DTISprites & \conftitle{ICCV} & 2021 & Transform Predictor & \EMPTY & \EMPTY & Reconstruction $L_2$ & \EMPTY & \EMPTY & \CHECK \\
EfficientMORL & \conftitle{ICML} & 2021 & Encoder/Decoder & Mask-based & Iterative & weighted ELBO & \EMPTY & \CHECK & \CHECK \\
GENESISv2 & \conftitle{NIPS} & 2021 & Encoder/Decoder & Mask-based & Iterative & GECO & \CHECK & \CHECK & \CHECK \\
GMAIR & \conftitle{CIN} & 2021 & Encoder/Decoder & Glimpse-based & Sequential & ELBO & \CHECK & \CHECK & \CHECK \\
GSNGs & \conftitle{ICLR} & 2021 & Encoder/Decoder & Glimpse-based & Sequential & ELBO & \CHECK & \CHECK & \CHECK \\
MarioNette & \conftitle{NIPS} & 2021 & Transform Predictor & \EMPTY & \EMPTY & Reconstruction $L_2$ & \CHECK & \EMPTY & \CHECK \\
uORF & \conftitle{ICLR} & 2022 & Encoder/Decoder & \EMPTY & Iterative & Reconstruction $L_2$ & \CHECK & \EMPTY & \CHECK \\ 
DINOSAUR & \conftitle{ICLR} & 2023 & Encoder/Decoder & Mask-based & Iterative & Reconstruction $L_2$  & \EMPTY & \EMPTY & \CHECK \\ \bottomrule
\end{tabular}%
}
\caption{Overview of decomposition methods and common techniques employed in UOD.}
\label{tab:overview_dec}
\end{table}

==> tables/table_overview_dec_a.tex <==
\let\conftitle\footnotesize

\begin{table}[]

\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule
\multicolumn{9}{c}{{\cellcolor{colordec}\textcolor{white}{{\textbf{Decomposition Methods}}}}} \\

%\multicolumn{9}{c}{\cellcolor{colordec}{\textcolor{white}{\textbf{\large Decomposition Methods}}}}                                 \\ \midrule
  Method &
  \begin{tabular}[c]{@{}c@{}}Pub.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Year\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Model\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Optimization\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Learning\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Attention\\Strategy\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Object\\Routing\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Reconstruction\end{tabular} \\ \midrule

AIR	& \conftitle{NIPS} & 2016 & VAE	& Variational Bayes	& ELBO	& Glimpse-based	& Sequential & STN-based \\
\rowcolor{rowbackground}
CST-VAE	& \conftitle{ICLR} 	& 2016	& VAE	& vVariational Bayes & ELBO	& Glimpse-based	& Sequential & STN-based \\
TAGGER & \conftitle{NIPS} & 2016 & Denoising AE & Backprop & NLL & Mask-based & Iterative & Fully Conntected \\
\rowcolor{rowbackground}
N-EM & \conftitle{NIPS} & 2017 & Recurrent AE & Backprop & Clustering & Mask-based & Iterative & CNN decoder \\
R-NEM & \conftitle{ICLR} & 2018 & Recurrent AE & Backprop & Clustering & Mask-based & Iterative & CNN decoder \\
\rowcolor{rowbackground}
SQAIR & \conftitle{NIPS} & 2018 & Recurrent VAE & Variational Bayes & IWAE & Glimpse-based & Sequential & Subpixel-CNN \\
GMIO & \conftitle{ICML} & 2019 & Encoder/Decoder &  & ELBO & Glimpse-based & Sequential &  \\
\rowcolor{rowbackground}
IODINE & \conftitle{ICML} & 2019 & VAE & Variational Bayes/IAI & weigthed ELBO & Mask-based & Iterative & Spatial broadcast \\
MONet & \conftitle{ARXIV} & 2019 & Recurrent VAE & Variational Bayes & ELBO+KL term & Mask-based & Sequential & Spatial broadcast \\
\rowcolor{rowbackground}
SCAE & \conftitle{NIPS} & 2019 & Capsule Autoencoder  & Backprop & Log-likelihood  & x & Template-based & Affine-transforms \\
SPAIR & \conftitle{AAAI} & 2019 & VAE & Variational Bayes & ELBO & Glimpse-based & Sequential & STN-based \\
\rowcolor{rowbackground}
SuPAIR & \conftitle{ICML} & 2019 & Sum-product Network &  & ELBO & Glimpse-based & Sequential &  \\
ECON  & \conftitle{ICLR} & 2020 & Encoder/Decoder &  & ELBO & Mask-based & Sequential &  \\
\rowcolor{rowbackground}
GENESIS & \conftitle{ICLR} & 2020 & Encoder/Decoder &  & GECO & Mask-based & Sequential &  \\
GNM & \conftitle{NIPS} & 2020 & Encoder/Decoder &  & ELBO & Glimpse-based & Sequential &  \\
\rowcolor{rowbackground}
LMIO & \conftitle{CVPR} & 2020 & Encoder/Decoder &  & IBL & Mask-based & Sequential &  \\
MulMON & \conftitle{NIPS} & 2020 & Encoder/Decoder &  & ELBO & Mask-based & Iterative &  \\
\rowcolor{rowbackground}
SCALOR & \conftitle{ICLR} & 2020 & Encoder/Decoder &  & ELBO & Glimpse-based & Sequential & \\ 
SLOT ATTENTION & \conftitle{NIPS} & 2020 & Differentiable interface &  & x & Mask-based & Iterative &  \\
\rowcolor{rowbackground}
SPACE & \conftitle{ICLR} & 2020 & Encoder/Decoder &  & ELBO & Glimpse-based & Sequential &  \\
SRN & \conftitle{NIPS} & 2020 & Differentiable interface &  & x & Mask-based & Iterative &  \\
\rowcolor{rowbackground}
DTISprites & \conftitle{ICCV} & 2021 & Transform Predictor &  & Reconstruction $L_2$ & x & x &  \\
EfficientMORL & \conftitle{ICML} & 2021 & Encoder/Decoder &  & weigthed ELBO & Mask-based & Iterative &  \\
\rowcolor{rowbackground}
GENESISv2 & \conftitle{NIPS} & 2021 & Encoder/Decoder &  & GECO & Mask-based & Iterative &  \\
GMAIR & \conftitle{CIN} & 2021 & Encoder/Decoder &  & ELBO & Glimpse-based & Sequential &  \\
\rowcolor{rowbackground}
GSNGs & \conftitle{ICLR} & 2021 & Encoder/Decoder &  & ELBO & Glimpse-based & Sequential &  \\
MarioNette & \conftitle{NIPS} & 2021 & Transform Predictor &  & Reconstruction $L_2$ & x & x &  \\
\rowcolor{rowbackground}
uORF & \conftitle{ICLR} & 2022 & Encoder/Decoder &  & Reconstruction $L_2$ & x & Iterative &  \\
DINOSAUR & \conftitle{ICLR} & 2023 & Encoder/Decoder & Backprop/Slot Attn. & Reconstruction $L_2$ & Mask-based & Iterative \\




 \bottomrule


\end{tabular}%
}
\caption{Overview of Decomposition methods with the most common techniques and characteristics.}
\label{tab:overview_dec}
\end{table}

==> tables/table_overview_seg.tex <==


\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lccccccc@{}}
\toprule
\multicolumn{8}{c}{Segmentation Methods}                        \\ \midrule
Method &
  \begin{tabular}[c]{@{}c@{}}Published \\ at\end{tabular} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Year\\ available\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}Employs \\ pseudo-masks\end{tabular} &
  Generative &
  \begin{tabular}[c]{@{}c@{}}Clustering\\ techniques\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Graph-based\\ techniques\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Code\\ availability\end{tabular} \\ \midrule
DC     & arxiv & 2010 & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \EMPTY \\
\rowcolor{rowbackground}
CoSand & arxiv & 2011 & \EMPTY    &       &       &       &       \\
IFBM   & arxiv & 2012 &         &       &       &       &       \\
\rowcolor{rowbackground}
MCC    & arxiv & 2012 &         &       &       &       &       \\
COMP   & arxiv & 2013 &         &       &       &       &       \\ 
\rowcolor{rowbackground}
CST     & arxiv & 2013 & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \EMPTY \\
HS     & arxiv & 2013 & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \EMPTY \\
\rowcolor{rowbackground}
OD     & arxiv & 2013 & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \EMPTY \\
GMS     & arxiv & 2014 & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \EMPTY \\
\rowcolor{rowbackground}
CS-ECEM     & arxiv & 2014 & \EMPTY & \EMPTY & \EMPTY & \CHECK & \EMPTY \\
SMD     & arxiv & 2014 & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \EMPTY \\
\rowcolor{rowbackground}
wCTR     & arxiv & 2014 & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \EMPTY \\
DMFC     & arxiv & 2015 & \EMPTY & \EMPTY & \EMPTY & \CHECK & \EMPTY \\
\rowcolor{rowbackground}
MRW     & arxiv & 2015 & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \EMPTY \\
WSC     & arxiv & 2015 & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \EMPTY \\
\rowcolor{rowbackground}
SCF     & arxiv & 2016 & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \EMPTY \\
CS-GSI     & arxiv & 2017 & \EMPTY & \EMPTY & \EMPTY & \CHECK & \EMPTY \\
\rowcolor{rowbackground}
SBF     & arxiv & 2017 & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \EMPTY \\
NPG     & arxiv & 2017 & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \EMPTY \\
\rowcolor{rowbackground}
SGC3     & arxiv & 2017 & \EMPTY & \EMPTY & \CHECK & \EMPTY & \EMPTY \\
CoAttnCNN     & arxiv & 2018 & \CHECK & \EMPTY & \EMPTY & \EMPTY & \EMPTY \\
\rowcolor{rowbackground}
DFF     & arxiv & 2018 & \EMPTY & \EMPTY & \CHECK & \EMPTY & \EMPTY \\
USD     & arxiv & 2018 & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \EMPTY \\
\rowcolor{rowbackground}
CP-GAN     & arxiv & 2019 & \EMPTY & \CHECK & \EMPTY & \EMPTY & \EMPTY \\
DeepCO3     & {\footnotesize CVPR} & 2019 & \CHECK & \EMPTY & \EMPTY & \EMPTY & \EMPTY \\
\rowcolor{rowbackground}
IIC     & arxiv & 2019 & \EMPTY & \EMPTY & \CHECK & \EMPTY & \EMPTY \\
REDO     & arxiv & 2019 & \EMPTY & \CHECK & \EMPTY & \EMPTY & \EMPTY \\
\rowcolor{rowbackground}
UnsupOD     & arxiv & 2020 & \CHECK & \EMPTY & \EMPTY & \EMPTY & \EMPTY \\
CS-OHS     & arxiv & 2021 & \EMPTY & \EMPTY & \EMPTY & \CHECK & \EMPTY \\
\rowcolor{rowbackground}
DeepUSPS     & arxiv & 2021 & \CHECK & \EMPTY & \EMPTY & \EMPTY & \EMPTY \\
DRC     & arxiv & 2021 & \EMPTY & \CHECK & \EMPTY & \EMPTY & \EMPTY \\
\rowcolor{rowbackground}
E-BigBiGAN     & arxiv & 2021 & \CHECK & \EMPTY & \EMPTY & \EMPTY & \EMPTY \\
MaskContrast     & arxiv & 2021 & \EMPTY & \EMPTY & \CHECK & \EMPTY & \EMPTY \\
\rowcolor{rowbackground}
PiCIE     & arxiv & 2021 & \EMPTY & \EMPTY & \CHECK & \EMPTY & \EMPTY \\
UVISAM     & arxiv & 2021 & \CHECK & \EMPTY & \EMPTY & \EMPTY & \EMPTY \\
\rowcolor{rowbackground}
DSM     & arxiv & 2022 & \EMPTY & \EMPTY & \EMPTY & \CHECK & \EMPTY \\
SegDiscover     & arxiv & 2022 & \CHECK & \EMPTY & \EMPTY & \EMPTY & \EMPTY \\
\rowcolor{rowbackground}
SegSwap     & arxiv & 2022 & \EMPTY & \EMPTY & \EMPTY & \EMPTY & \EMPTY \\
SelfMask     & arxiv & 2022 & \CHECK & \EMPTY & \EMPTY & \EMPTY & \EMPTY \\
\rowcolor{rowbackground}
TokenCut     & arxiv & 2022 & \CHECK & \EMPTY & \EMPTY & \CHECK & \CHECK \\





 
\bottomrule
\end{tabular}%
}
\caption{Overview of segmentation methods and common techniques employed in UOD.}
\label{tab:overview_seg}
\end{table}

==> tables/table_overview_seg_a.tex <==
\let\conftitle\footnotesize

\begin{table}[]

\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
\multicolumn{11}{c}{\cellcolor{colorseg}{\textcolor{white}{\textbf{Segmentation Methods}}}}                                 \\ \midrule
  Method &
  \begin{tabular}[c]{@{}c@{}}Pub.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Year\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Model\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Optimization\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Representation\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Learning\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}External saliency\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Oversegmentation\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Clustering\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Mask\\Generation\end{tabular} \\ \midrule

DC & \conftitle{ICML} & 2010 & Semidefinite program & Low-rank op. & Hand-crafted & x & x & Watershed & Discrim./Spectral & Threshold \\

\rowcolor{rowbackground}
CoSand	& \conftitle{ICCV} & 2011 & Temperature maximization & Submodular op.+Ncut & Hand-crafted & x & x & Superpixels & Spectral & \EMPTY \\	

IFBM & \conftitle{CVPR} & 2012 & MRF-based & Graph cuts & Hand-crafted & x & x & Mean-shift & GMM/Spectral & \EMPTY \\

\rowcolor{rowbackground}
MCC	& \conftitle{CVPR} & 2012 & Combinatorial pixel labeling & Block-coord. descent & Hand-crafted & x & x & Superpixels & Discrim./Spectral & \EMPTY \\	

COMP & \conftitle{ICCV} & 2013 & Score-based refinement & Heuristic seg.+Grabcut & Hand-crafted & x & Likelihood maps & x & x & Label assign. \\

\rowcolor{rowbackground}
CST & \conftitle{ICCV} & 2013 & MRF-based & Graph cuts & Hand-crafted & x & x & x & \EMPTY \\

HS	& \conftitle{CVPR} & 2013 & Tree-structure graphical & Belief propagation & Hand-crafted & x & x & Watershed & x & Saliency fusion \\

\rowcolor{rowbackground}
OD	& \conftitle{CVPR} & 2013 & Pixel correspondence optim. & Coordinate descent & Hand-crafted & x & Contrast-based saliency & x & x & Refinement \\

GMS	& \conftitle{ICIP} & 2014 & Global saliency fusion & Grabcut & Hand-crafted & x	& Contrast-based saliency & Superpixels & K-means & Label assign. \\

\rowcolor{rowbackground}
CS-ECEM	& \conftitle{TCSVT} & 2014 & Superpixel labelling & \(\alpha\)-Expansion algorithm & Hand-crafted & x & Objectness estimation & Superpixels & Affinity propagation & \EMPTY \\

SMD	& \conftitle{TPAMI} & 2017 & Structured matrix decomp. & Felzenszwalb algorithm & Hand-crafted & x & Sparse/Dense reconstr. & Superpixels & x & Context propag. \\

\rowcolor{rowbackground}
wCTR & \conftitle{CVPR} & 2014 & Graph-based approach & Least-square op. & Hand-crafted & x & Contrast-based saliency & Superpixels & x & Label assign. \\

DMFC & \conftitle{CVIU} & 2015 & Graph-based approach & Alternating op./Grabcut & Hand-crafted & x & Probability-based saliency & Superpixels & GMM & Threshold \\

\rowcolor{rowbackground}
MRW & \conftitle{CVPR} & 2015 & Graph-based approach & Random walkers & Hand-crafted & x & x & Superpixels & MRW-based & Bilateral filter \\

WSC & \conftitle{CVPR} & 2015 & Dictionary-based saliency & Sparse coding & Hand-crafted & x & x & Superpixels & x & Threshold \\

\rowcolor{rowbackground}
SCF & \conftitle{TMM} & 2016 & Quadratic programming & Grabcut & Hand-crafted & x & Multiple methods & Superpixels & K-means & Label assign. \\

SBF & \conftitle{ICCV} & 2017 & Saliency network & Backprop & Learned & Fused weak saliency & Multiple methods & Superpixels & x & \EMPTY \\	

\rowcolor{rowbackground}
NPG & \conftitle{TIP} & 2017 & Mixed-Integer Programs & Grabcut & Learned & x & Segmentation map & Hierarchical mrg. & x & Label assign. \\

SGC3 & \conftitle{AAAI} & 2017 & Constrained clustering & K-means like optim. & Hand-crafted & x & Adaptive threshold & Superpixels & Cosine sim. based & Cluster assign. \\

\rowcolor{rowbackground}
CoAttCNN & \conftitle{IJCA} & 2018 & Two-stage optimization & Backprop & Pretrained & Off-the-shelf proposals & CNN feature map & x & x & CRF \\

CS-GSIN & \conftitle{NEUCOM} & 2018 & Tree structure graph & Grabcut & Hand-crafted & x & Saliency tree & Gpb-owt-ucm & K-means & Label assign. \\

\rowcolor{rowbackground}
DFF & \conftitle{ECCV} & 2018 & Non-negative Factorization & Low-rank approx. & Pretrained & x & CNN feature map & x & NMF & Threshold \\

USDNL & \conftitle{CVPR} & 2018 & Saliency network & Backprop & Learned & Off-the-shelf saliency & Multiple methods & x & x & \EMPTY \\

\rowcolor{rowbackground}
CP-GAN & \conftitle{ARXIV} & 2019 & GAN & Backprop & Learned & Adversarial & x & x & x & Composition \\

DeepCO3 & \conftitle{CVPR} & 2019 & Multi-loss optimization & Backprop & Refined & Feat. Corr./Saliency & Off-the-shelf & x & x & Proposal ranking \\

\rowcolor{rowbackground}
IIC & \conftitle{ICCV} & 2019 & Clustering neural network & Backprop & Learned & Mutual inform. & x & Overclustering & Soft clustering & \EMPTY \\

ReDo & \conftitle{NIPS} & 2019 & GAN & Backprop & Learned & Aversarial & x & x & x & Composition \\

\rowcolor{rowbackground}
DeepUSPS & \conftitle{NIPS} & 2019 & Saliency network & Backprop & Learned & Pseudo-labels & Handcrafted saliency & x & x & CRF \\

UnsupOD & \conftitle{SYMM.} & 2020 & Segmentation network & Backprop & Learned & Img. reconstruction & x & x & x & \EMPTY \\

\rowcolor{rowbackground}
CS-OHS & \conftitle{JCS} & 2021 & MRF-based & Particle Swarm & Hand-crafted & x & DL saliency method & Superpixels & x & \EMPTY \\	

DRC & \conftitle{NIPS} & 2021 & Generative modeling - MoE & EM-like/MCMC/Bprop & Learned & Img. reconstruction & x & x & x & \EMPTY \\

\rowcolor{rowbackground}
E-BigBigGAN & \conftitle{PMLR} & 2021 & Segmentation network & Backprop & Refined & Synthetic masks & Latent space guided & x & x & \EMPTY \\

MaskContrast & \conftitle{ICCV} & 2021 & Pixel-embedding learning & Backprop & Learned & Contrastive & DL saliency method & x & K-means & \EMPTY \\

\rowcolor{rowbackground}
PiCIE & \conftitle{CVPR} & 2021 & Pixel-embedding learning & Backprop & Refined & Cluster assignments & x & x & K-means	& \EMPTY \\

UVISAM & \conftitle{BMVC} & 2022 & Segmentation network & Backprop & Refined & Optical flow & x & x & x & \EMPTY \\

\rowcolor{rowbackground}
DSM & \conftitle{CVPR} & 2022 & Graph-based Spectral & Normalized cut & Pretrained & x & Tranformer Feat. map & Overclustering & Spectral/k-means & CRF \\

MOVE & \conftitle{NIPS} & 2022 & Segmenter/inpainter net. & Bprop/Adversarial tr. & Pretrained & composite image & Tranformer Feat. map & x & x & Segmenter \\

\rowcolor{rowbackground}
SegDiscover & \conftitle{ARXIV} & 2022 & Segmentation network & Backprop & Refined & Cluster assignments & x &	Superpixels & K-means/Spectral & \EMPTY \\

SegSwap & \conftitle{CVPR} & 2022 & Graph-based Pair Matching & Grabcut & Pretrained & Correspondence pairs & LOST/bilateral solver & x & K-means & Label assign. \\

\rowcolor{rowbackground}
SelfMask & \conftitle{CVPRw} & 2022 & Saliency network & Backprop & Learned & Ranked saliency mask & CNN/Transf. feat. maps & x & Spectral & Threshold \\

TokenCut & \conftitle{CVPR} & 2022 & Graph-based Spectral & Normalized cut & Pretrained & x & Tranformer Feat. map & x & Spectral & Threshold \\

\rowcolor{rowbackground}
CutLER & \conftitle{CVPR} & 2023 & Segmentation network & Ncut/Backprop & Pretrained & MaskCut pseudo-labels & Tranformer Feat. map & x & x & Decoder \\

SEMPART & \conftitle{ICCV} & 2023 & Graph-based approach & Backprop & Refined & Coarse/fine bi-partition & Tranformer Feat. map & x & x & Sal. refinement \\

\rowcolor{rowbackground}
U2Seg & \conftitle{CVPR} & 2024 & Segmentation network & EM/Backprop & Refined & Pseudo-labels & CutLer/Stego & Maskcut masks & K-means & Decoder  \\


 \bottomrule


\end{tabular}%
}
\caption{Overview of Segmentation methods and common techniques employed in UOD.}
\label{tab:overview_dec}
\end{table}

==> tables/table_overview_seg_b.tex <==
\let\conftitle\footnotesize

\begin{table}[]
\centering
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{@{}lccccccccc@{}}
\toprule
\multicolumn{10}{c}{\cellcolor{colorseg}{\textcolor{white}{\textbf{Segmentation Methods}}}}                                 \\ \midrule
  Method &
  \begin{tabular}[c]{@{}c@{}}Pub.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Year\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Intra-img sim.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Inter-img sim.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Probabilistic \\ formulations\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Graph-based \\ techniques\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Generative \\ modeling\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Deep \\ learning\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Code \\ released\end{tabular} \\ \midrule

DC & \conftitle{ICML} & 2010 & \CHECK &	\CHECK & x & \CHECK & x & x	& \CHECK \\

\rowcolor{rowbackground}
CoSand	& \conftitle{ICCV} & 2011 & \CHECK & \CHECK & x & \CHECK & x & x & \CHECK \\	

IFBM & \conftitle{CVPR} & 2012 & \CHECK & \CHECK & \CHECK &	\CHECK & \CHECK & x & x \\

\rowcolor{rowbackground}
MCC	& \conftitle{CVPR} & 2012 & \CHECK & \CHECK & \CHECK & \CHECK &	x & x & \CHECK \\	

COMP & \conftitle{ICCV} & 2013 & \CHECK & \CHECK & \CHECK &	\CHECK & x & x & \CHECK \\

\rowcolor{rowbackground}
CST & \conftitle{ICCV} & 2013 & \CHECK & \CHECK & \CHECK & \CHECK &	x & x & \CHECK \\

HS	& \conftitle{CVPR} & 2013 & \CHECK & x & x & x & x & x & x \\

\rowcolor{rowbackground}
OD	& \conftitle{CVPR} & 2013 & \CHECK & \CHECK & x & x & x & x	& \CHECK \\

GMS	& \conftitle{ICIP} & 2014 & \CHECK & \CHECK & x & \CHECK & x & x & \CHECK \\

\rowcolor{rowbackground}
CS-ECEM	& \conftitle{TCSVT} & 2014 & \CHECK & \CHECK & x & \CHECK & x & x & x \\

SMD	& \conftitle{TPAMI} & 2017 & \CHECK & x & x & \CHECK & x & x & x \\

\rowcolor{rowbackground}
wCTR & \conftitle{CVPR} & 2014 & \CHECK & x & x & \CHECK & x & x & \CHECK \\

DMFC & \conftitle{CVIU} & 2015 & \CHECK & \CHECK & \CHECK &	\CHECK & x & x & \CHECK \\

\rowcolor{rowbackground}
MRW & \conftitle{CVPR} & 2015 & \CHECK & \CHECK & \CHECK & \CHECK &	x & x & x \\

WSC & \conftitle{CVPR} & 2015 & \CHECK & x & x & \CHECK & x & x & \CHECK \\

\rowcolor{rowbackground}
SCF & \conftitle{TMM} & 2016 & x & \CHECK &	x & \CHECK & x & x & \CHECK \\

SBF & \conftitle{ICCV} & 2017 & x & x & \CHECK & x & x & \CHECK & \CHECK \\	

\rowcolor{rowbackground}
NPG & \conftitle{TIP} & 2017 & x & \CHECK &	\CHECK & \CHECK & x & \CHECK & x \\

SGC3 & \conftitle{AAAI} & 2017 & x & \CHECK & x & x & x & x & x \\

\rowcolor{rowbackground}
CoAttCNN & \conftitle{IJCA} & 2018 & x & \CHECK & x & x & x & \CHECK & x \\

CS-GSI & \conftitle{NEUCOM} & 2018 & \CHECK & \CHECK & x & \CHECK & x & x & x \\

\rowcolor{rowbackground}
DFF & \conftitle{ECCV} & 2018 & x & \CHECK & x & x & x & \CHECK & \CHECK \\

USDNL & \conftitle{CVPR} & 2018 & x & x & \CHECK & x & x & \CHECK & x \\

\rowcolor{rowbackground}
CP-GAN & \conftitle{ARXIV} & 2019 & x & x & \CHECK & x & \CHECK & \CHECK & x \\

DeepCO3 & \conftitle{CVPR} & 2019 & x & \CHECK & x & x & x & \CHECK & \CHECK \\

\rowcolor{rowbackground}
IIC & \conftitle{ICCV} & 2019 & \CHECK & x & \CHECK & x & x & \CHECK & \CHECK \\

ReDo & \conftitle{NIPS} & 2019 & x & x & \CHECK & x & \CHECK & \CHECK & x \\

\rowcolor{rowbackground}
DeepUSPS & \conftitle{NIPS} & 2019 & x & x & x & x & x & \CHECK & \CHECK \\

UnsupOD & \conftitle{SYMM.} & 2020 & x & x & x & x & x & \CHECK & x \\

\rowcolor{rowbackground}
CS-OHS & \conftitle{JCS} & 2021 & x & \CHECK & x & x & x & \CHECK &	x \\	

DRC & \conftitle{NIPS} & 2021 & x & x & \CHECK & x & \CHECK & \CHECK & \CHECK \\

\rowcolor{rowbackground}
E-BigBigGAN & \conftitle{PMLR} & 2021 & x & x & x & x & x & \CHECK & \CHECK \\

MaskContrast & \conftitle{ICCV} & 2021 & \CHECK & \CHECK & x & x & x & \CHECK &	\CHECK \\

\rowcolor{rowbackground}
PiCIE & \conftitle{CVPR} & 2021 & x & \CHECK & x & x & x & \CHECK &	\CHECK \\

UVISAM & \conftitle{BMVC} & 2022 & x & x & x & x & x & \CHECK &	\CHECK \\

\rowcolor{rowbackground}
DSM & \conftitle{CVPR} & 2022 & \CHECK & \CHECK & x & \CHECK & x & \CHECK &	\CHECK \\

MOVE & \conftitle{NIPS} & 2022 & \CHECK & x & x & x & x & \CHECK & \CHECK \\

\rowcolor{rowbackground}
SegDiscover & \conftitle{ARXIV} & 2022 & x & \CHECK & x & x & x & \CHECK & x \\

SegSwap & \conftitle{CVPR} & 2022 & x & \CHECK & x & \CHECK & x & \CHECK & \CHECK \\

\rowcolor{rowbackground}
SelfMask & \conftitle{CVPRw} & 2022 & \CHECK & x & x & x & x & \CHECK &	\CHECK \\

TokenCut & \conftitle{CVPR} & 2022 & \CHECK & x & x & \CHECK &	x & \CHECK & \CHECK \\

\rowcolor{rowbackground}
CutLER & \conftitle{CVPR} & 2023 & \CHECK & x & x & \CHECK & x & \CHECK & \CHECK \\

SEMPART & \conftitle{ICCV} & 2023 & \CHECK & x & x & \CHECK & x & \CHECK & x \\

\rowcolor{rowbackground}
U2Seg & \conftitle{CVPR} & 2024 & \CHECK & \CHECK & x & x & x & \CHECK & \CHECK \\


 \bottomrule


\end{tabular}%
}
\caption{Overview of Segmentation methods and common techniques employed in UOD.}
\label{tab:overview_dec}
\end{table}

==> tables/table_singleloc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lccccccc@{}}
\toprule
\multirow{2}{*}{Methods} &
  \multirow{2}{*}{\textbf{Year}} &
  \multicolumn{1}{l}{\textbf{Object   Discovery}} &
  \multicolumn{1}{l}{\textbf{PASCAL07-6x2}} &
  \multicolumn{1}{l}{\textbf{PASCAL07-All}} &
  \multicolumn{1}{l}{\textbf{PASCAL VOC 2012}} &
  \multicolumn{1}{l}{\textbf{ImageNet Subsets}} &
  \multicolumn{1}{l}{\textbf{COCO\_20k}} \\ \cmidrule(l){3-8} 
            &      & \multicolumn{6}{c}{CorLoc}                                                  \\ \midrule
CoLocFW \textsuperscript{\tsa}   & 2014 & -           & -           & 24.59       & -           & -     & -           \\
CoLocRWI \textsuperscript{\tsa}  & 2014 & 76.58       & 39.31       & -           & -           & -     & -           \\
UODLWild    & 2015 & 82.35       & 53.73       & 31.30       & -           & -     & -           \\
CoLocCSD \textsuperscript{\tsa}  & 2016 & -           & -           & 40.0        & 43.80       & 48.30 & -           \\
DDT \textsuperscript{\tsa}       & 2017 & 88.13       & -           & 46.90       & 49.40       & 69.10 & -           \\
CoLocGDP \textsuperscript{\tsa}  & 2019 & 85.67       & -           & 41.20       & 47.45       & 63.50 & -           \\
OSD         & 2019 & 83.0 ± 0.40 & 60.2 ± 0.40 & 39.8 ± 0.20 & -           & -     & -           \\
UODSphClust & 2019 & 89.40       & -           & 49.50       & -           & 77.60 & -           \\
OLM         & 2020 & 85.80       & 58.29       & 37.90       & -           & 60.10 & -           \\
rOSD        & 2020 & 89.2 ± 0.40 & 72.5 ± 0.50 & 49.3 ± 0.20 & 51.2 ± 0.20 & -     & 48.5 ± 0.10 \\
LOD         & 2021 & -           & -           & 48.0        & 50.50       & -     & 48.50       \\
LOST        & 2021 & -           & -           & 54.90       & 57.50       & -     & 57.50       \\ \bottomrule
\end{tabular}%
}
\caption{Comparison of single-object localization methods in terms of reported average CorLoc. \tsa method runs on single-class dataset.}
\label{tab:singleloc}
\end{table}
